Robotic Vision for Human-Robot Interaction and Collaboration: A Survey and Systematic Review

Robotic vision for human-robot interaction and collaboration is a critical process for robots to collect and interpret detailed information related to human actions, goals, and preferences, enabling robots to provide more useful services to people. This survey and systematic review presents a comprehensive analysis on robotic vision in human-robot interaction and collaboration over the last 10 years. From a detailed search of 3850 articles, systematic extraction and evaluation was used to identify and explore 310 papers in depth. These papers described robots with some level of autonomy using robotic vision for locomotion, manipulation and/or visual communication to collaborate or interact with people. This paper provides an in-depth analysis of current trends, common domains, methods and procedures, technical processes, data sets and models, experimental testing, sample populations, performance metrics and future challenges. This manuscript found that robotic vision was often used in action and gesture recognition, robot movement in human spaces, object handover and collaborative actions, social communication and learning from demonstration. Few high-impact and novel techniques from the computer vision field had been translated into human-robot interaction and collaboration. Overall, notable advancements have been made on how to develop and deploy robots to assist people.

==> ExtraFiles/scratchpad.tex <==
All papers related to gesture recognition are listed here: ~\cite{luo_tracking_2011,milligan_selecting_2011,lichtenstern_prototyping_2012, nishiyama_human_2013, alonso-mora_human_2014, canal_gesture_2015, fareed_gesture_2015, song_towards_2017,lima_real-time_2019, martin_real-time_2019, zhang_interactive_2018, chen_human-following_2019, miller_self-driving_2019, droeschel_towards_2011, canal_gesture_2015, moh_gesture_2019, sriram_mobile_2019, kalidolda_towards_2018,paulo_vision-based_2012,lam_real-time_2011, cicirelli_kinect-based_2015,fareed_gesture_2015,lalejini_evaluation_2015, ghandour_human_2017, long_kinect-based_2018,pentiuc_drive_2018, zhang_interactive_2018,chen_human-following_2019, miller_self-driving_2019, li_real-time_2019, chen_approaches_2010,manigandan_wireless_2010,faudzi_real-time_2012, lavanya_gesture_2018, waskito_wheeled_2020, xu_skeleton_2020,park_real-time_2011, van_den_bergh_real-time_2011, yoshida_evaluation_2011, abidi_human_2013, prediger_robot-supported_2014, chen_stereovision-only_2014, jevtic_comparison_2015, tolgyessy_foundations_2017,wang_wheeled_2013,fang_vehicle-mounted_2019,fujii_gesture_2014,ghandour_human_2017,yoshida_evaluation_2011,mao_medical_2018} (Only half done). 
\\
Test for importing citations:
\\
\cite{arumbakkam_multi-modal_2010,budiharto_indoor_2010,chen_integrated_2010,chen_approaches_2010,couture-beil_selecting_2010,fahn_real-time_2010,kobayashi_people_2010,manigandan_wireless_2010,martin_estimation_2010,sisbot_synthesizing_2010,sosnowski_mirror_2010,yun_robust_2010,tan_safety_2010,droeschel_towards_2011,luo_human_2010,masmoudi_expressive_2011,broccia_gestural_2011,ding_optimizing_2011,igorevich_behavioral_2011,jia_autonomous_2011,lam_real-time_2011,luo_tracking_2011,milligan_selecting_2011,nair_3d_2011,park_real-time_2011,saegusa_cognitive_2011,van_den_bergh_real-time_2011,yoshida_evaluation_2011,alvarez-santos_feature_2012,burger_two-handed_2012,chen_person_2012,cheng_design_2012,csapo_multimodal_2012,faudzi_real-time_2012,foster_two_2012,gori_all_2012,lambrecht_spatial_2012,lichtenstern_prototyping_2012,mead_probabilistic_2012,paulo_vision-based_2012,stipancic_programming_2012,torres_implementation_2012,wu_accompanist_2012,bdiwi_handing-over_2013,abidi_human_2013,cheng_multiple-robot_2013,ferrer_robot_2013,indrajit_development_2013,nishiyama_human_2013,pereira_human-robot_2013,qian_visually_2013,tao_multilayer_2013,wang_vision-guided_2013,wang_wheeled_2013,weinrich_appearance-based_2013,werner_evaluation_2013,yang_study_2013,yun_robotic_2013,alonso-mora_human_2014,castellano_context-sensitive_2014,chen_stereovision-only_2014,do_human-robot_2014,fujii_gesture_2014,hu_design_2014,miyoshi_above_2014,morato_toward_2014,munaro_fast_2014,nguyen_audio-visual_2014,petric_online_2014,prediger_robot-supported_2014,scheggi_human-robot_2014,shieh_fuzzy_2014,taheri_social_2014,tseng_multi-human_2014,xu_online_2014,ali_improved_2015,canal_gesture_2015,cech_active-speaker_2015,cherubini_unified_2015,choudhary_real_2015,cicirelli_kinect-based_2015,fareed_gesture_2015,gao_humanoid_2015,gupta_robust_2015,jevtic_comparison_2015,katsuki_high-speed_2015,lalejini_evaluation_2015,li_visual_2015,quintero_visual_2015,saleh_nonverbal_2015,vircikova_teach_2015,yang_real-time_2015,bayram_audio-visual_2016,christiernin_interacting_2016,ehlers_human-robot_2016,hassan_computationally_2016,ikai_robot_2016,kahily_real-time_2016,ke_vision_2016,koppula_anticipating_2016,koustoumpardis_human_2016,mollaret_multi-modal_2016,moreno_path_2016,potdar_learning_2016,ratul_gesture_2016,talebpour-board_2016,vasconcelos_socially_2016,vaufreydaz_starting_2016,zhang_optimal_2016,angonese_multiple_2017,arenas_deep_2017,bellarbi_social_2017,bilac_gaze_2017,deepan_raj_static_2017,dometios_real-time_2017,ghandour_human_2017,gorer_autonomous_2017,han_human_2017,ju_integrative_2017,lee_learning_2017,maurtua_natural_2017,meghdari_real-time_2017,shariatee_safe_2017,song_towards_2017,tolgyessy_foundations_2017,wang_collision-free_2017,yao_monocular_2017,yoo_gaze_2017,zhu_robust_2017,vasquez_deep_2017,araiza-lllan_dynamic_2018,bolano_towards_2018,bothe_effective_2018,du_online_2018,efthymiou_multi-_2018,gong_research_2018,gui_teaching_2018,hong_interactive_2018,kalidolda_towards_2018,lavanya_gesture_2018,li_learning_2018,long_kinect-based_2018,mao_medical_2018,pasinetti_development_2018,pentiuc_drive_2018,sorostinean_activity_2018,weber_follow_2018,yuan_development_2018,zhang_indoor_2018,zhang_interactive_2018,zhang_automating_2018,cazzato_real-time_2019,chalvatzaki_learn_2019,chen_wristcam_2019,chen_human-following_2019,chien_navigating_2019,condes_person_2019,fang_vehicle-mounted_2019,haghighi_integration_2019,jarosz_detecting_2019,kogkas_free-view_2019,landi_prediction_2019,li_inferring_2019,li_real-time_2019,li_cnn_2019,lima_real-time_2019,luo_human-robot_2019,luo_real-time_2019,martin_real-time_2019,mazhar_real-time_2019,miller_self-driving_2019,moh_gesture_2019,scimmi_experimental_2019,sriram_mobile_2019,valle_personalized_2019,vysocky_interaction_2019,wu_improved_2019,yang_socially-aware_2019,zardykhan_collision_2019,zhang_vision-based_2019,anuradha_human_2020,augello_towards_2020,avioz-sarig_robotic_2020,bingol_practical_2020,chan_collision-free_2020,ferraguti_safety_2020,gao_hand_2020,hwang_interactions_2020,lang_research_2020,lee_visual_2020,lee_real-time_2020,liu_dynamic_2020,lu_research_2020,mronga_constraint-based_2020,phong_vietnamese_2020,tarbouriech_bi-objective_2020,van_den_broek_ergonomic_2020,waskito_wheeled_2020,wu_toward_2020,xu_skeleton_2020,yuan_natural_2020,zhang_human_2020,gao_user_2020,almonfrey_flexible_2018,monajjemi_hri_2013,jindai_small-size_2010,hasanuzzaman_adaptation_2010,mendez-polanco_detection_2010,weiss_robots_2010,pustianu_mobile_2011,sanna_kinect-based_2012,celik_development_2012,gu_human_2012,lee_human_2012,de_luca_integrated_2012,lee_interactive_2012,konda_real_2012,li_cyber-physical_2013,cid_real_2013,das_attracting_2013,schmidt_contact-less_2013,pfeil_exploring_2013,hartmann_feasibility_2013,granata_human_2013,zhao_interactive_2013,anzalone_multimodal_2013,hegger_people_2013,moe_real-time_2013,baron_remote_2013,ozgur_natural_2014,costante_personalizing_2014,barros_real-time_2014,farulla_real-time_2014,chao_robotic_2014,saveriano_safe_2014,batista_probabilistic_2015,nazari_simplified_2015,zhang_adaptive_2015,saffar_context-based_2015,saichinmayi_gesture_2015,benabdallah_kinect-based_2015,obo_robot_2015,voisan_ros-based_2015,fuad_skeleton_2015,monajjemi_uav_2015,nagi_wisdom_2015,guo_control_2016,simul_support_2016,liu_interactive_2016,maraj_application_2016,manitsaris_fingers_2016,mateus_human-aware_2016,li_id-match_2016,silva_mirroring_2016,zambelli_multimodal_2016,zhu_real-time_2016,agrigoroaie_enrichme_2016,vignolo_computational_2017,barz_evaluating_2017,valipour_incremental_2017,maher_realtime_2017,rehman_target_2017,devanne_co-design_2018,shakev_autonomous_2018,lathuiliere_deep_2018,bras_gesture_2018,mohaimenianpour_hands_2018,costanzo_multimodal_2019,azari_commodifying_2019,yu_efficiency_2019,belo_facial_2019,yu_interactive_2019,paetzel_let_2019,chen_online_2019,svarny_safe_2019,ali_smart_2019,gemerek_video-guided_2019,sun_visual_2019,muller_multi-modal_2020,kawasaki_multimodal_2020,yan_optimization_2020,sanchez-matilla_benchmark_2020,nascimento_collision_2020,fallahinia_comparison_2020,chen_design_2020,pang_efficient_2020,angani_human_2020,medeiros_human-drone_2020,yue_human-robot_2020,terreran_low-cost_2020,hsu_real-time_2020,de_schepper_towards_2020,uribe_mobile_2011,hafiane_3d_2013,mohammad_tele-operation_2013,xiao_human-robot_2014,quintero_interactive_2014,zhao_intuitive_2016,bouteraa_gesture-based_2017,bai_kinect-based_2018,abiddin_development_2019,sripada_teleoperation_2019}



%This is instead in the graph above - Gesture recognition was paired with different camera systems: depth aware cameras ($N=54$, Microsoft Kinect ($N=48$)), single camera set-ups ($N=21$), stereo cameras ($N=4$), and omni-directional cameras ($N=1$). 
%Gestures often involved pointing ($N=24$, ~\cite{martin_estimation_2010, luo_tracking_2011, milligan_selecting_2011, abidi_human_2013, prediger_robot-supported_2014,jevtic_comparison_2015, maurtua_natural_2017, tolgyessy_foundations_2017}), making a fist ($N=13$), waving ($N=8$, ~\cite{couture-beil_selecting_2010, cheng_design_2012,tao_multilayer_2013, fujii_gesture_2014,canal_gesture_2015}), finger count ($N=11$), thumbs up ($N=3$,  ~\cite{manigandan_wireless_2010, faudzi_real-time_2012, vysocky_interaction_2019}), 'stop' signal~\cite{faudzi_real-time_2012, ehlers_human-robot_2016} and other gestures ($N=21$, including gestures from body pose). 




Identified domains included manufacturing and warehouses, field (e.g. human-robot teaming /  human-supervisor [operator] - include above or below ground/water, indoor/domestic, (e.g. social robots, humanoid robots)

Application areas: Handling, Welding, Assembly 
RV Techniques: Image Processing, Feature Detection, Segmentation, 

Introduction to the concept and topic. What is it, why is it important, papers that describe gesture recognition (with or without robot). 
What are some of the main use cases or domain areas that gesture recognition is used - (Operation and Communication). 
This stage can include papers that are broader in domain. Mention some reviews but briefly if they are older than 10 years. 
1-3 sentences per paper at this stage (unless the paper is highly comprehensive and describes exactly what you want to say, then feel free to add more than 3). 

What are the differences between state of the art from computer vision conferences (for example) and what is being used in HRC to date? 
How can this be improved to make better robots that can utilize gesture recognition? 


Kinesics (Movements: Actions, Facial Macro, Facial Micro, Proxemics (Distance), Haptics (Touch), Emotion (Recognition), Chronemics (Time). 

Six people with different heights performed 5 gestures 50 times each~\cite{han_human_2017}. 

From the total 1500 gestures, there were 11 errors, with no significance in accuracy between short, medium and tall people. 

Five people with different heights perform gestures to control a mobile robot~\cite{ghandour_human_2017}. In the total 90 gestures issued, two were misclassified~\cite{ghandour_human_2017}. From the failures, 78.9\% were related to distance and rotational speed of the robot. 


Task type was identified as a high level overview (i.e. walking assistant, search and rescue, etc). Task criticality referred to when failure could affect the life of a person, and it was divided into three categories: high, medium and low. Robot morphology was classified as physical appearance based on three categories: anthropomorphic (i.e. human-like), zoomorphic (i.e. animal-like) and functional (i.e. neither, but focusing on the function of the robot). Ratio of robot to people was calculated the number of humans over the number of robots. Composition of robot teams involved whether robot teams contained the same or different type of robot, classified as homogeneous or heterogeneous. Level of shared interaction among teams involved the formation of the human-robot team. Interaction role was one of the five following classifications: supervisor, operator, mechanic/programmer, teammate and bystander. Type of human-robot physical proximity included passing, following, avoiding, approaching, touching and none of the above. Space/time taxonomy classified if robots and humans were used at different times (asynchronus), same time (synchronous), while in the same location (collocated) or different location (non-collocated) \cite{yanco2004classifying}. Level of robot autonomy in HRI/C reported using \cite{beer2014toward}'s 10-point taxonomy: 1) manual teleoperation, 2) action support, 3) assisted teleoperation, 4) batch processing, 5) decision support, 6) shared control with human initiative, 7) shared control with robot initiative, 8) supervisory control, 9) executive control, and 10) full autonomy.

==> ExtraFiles/scratchpad_TackActionGestureBackup.tex <==
\subsubsection{Task/Action of the Robot:}

% ARMS ====================================
A small robot arm with a gripper identifies when a persons hand is open, and moves to drop a small object into the users palm~\cite{arenas_deep_2017}. When the persons hand is closed the robot returns to its initial position.

A WAM robot arm (7DOF) makes a pizza following human direction to by moving ingredients that are pointed at by the human~\cite{quintero_visual_2015}. The human point to an object, the robot confirms the location the object by also pointing (robot to human feedback). The human performs a confirmation gesture and instructs the robot to drop the ingredients over the pizza base. 

An industrial robot arm tracks hand position with a Kinect sensor and an inertial measurement unit (IMU) worn by the user, while learning from online demonstrations~\cite{du_online_2018}. When the robot end effector gets close to the desired position, fine tuning is performed by speech and static hand gesture pointing.

The tool centre point of an industrial arm moves in front of a work piece to be machined, as pointed to by a human operator~\cite{maurtua_natural_2017}. 

A robot equipped with two arms, stereo vision, and tactile sensors picks up an object (sponge cube, wooden cube, ping-pong ball) determined by a hand pointing gesture from a human operator~\cite{ikai_robot_2016}. The robot releases the object on the palm of the operator.

% Mobile ====================================
A spherical vision system is used with a mobile robot with three omni-directional wheels to detect pointing gestures from a person wearing a red coat with a blue glove ~\cite{yoshida_evaluation_2011}. The robot moves on a soccer field in the direction of the pointing gesture.

The velocity of a wheelchair robot was commanded by human shoulder position, and its configuration was controlled with arm gestures (transitioning between bed mode and sitting mode)~\cite{mao_medical_2018}. 

A autonomous mobile navigation robot explores a laboratory, asking humans for directions (when a human is detected) and translating hand gesture pointing to goals on the robot's map~\cite{van_den_bergh_real-time_2011}.

A mobile robot with a manipulator named Jido responds to gestures that involve both hands, and user speech, to identify, fetch, and handover objects (such as a water bottle)~\cite{burger_two-handed_2012}. 

A team of four mobile robots respond to gestures from a human operator~\cite{milligan_selecting_2011}. The operator selects a group of robots at a time by drawing a circle around the desired group. A robot is selected if the operators face is detected within the cone created by the circle gesture. The selected robots then go to a location pointed to by the operator. Each robot has an LED to provide feedback when the robots are searching for the operator's face, and when they are selected.

% Social ====================================
A humanoid exercise robot (NAO and Poppy) demonstrated a pose for a human to perform and provide feedback on the quality of the exercise~\cite{avioz-sarig_robotic_2020}. The robot keeps track of the number of exercises correctly performed, changing to a new exercises when the user raises their hand. Elderly users were motivated to exercise by the interaction.

Body pose (for example arms out front, or above the persons head) was used to command a swarm of small mobile robots to move into a set configuration (such as making a smiling face)~\cite{alonso-mora_human_2014}. 

A mobile social robot determines the appropriate time to approach a human after inferring user intent through body gestures and facial expressions~\cite{li_inferring_2019}. For these demonstrations there is often more than one human in the robot field of view, and the robot must at all times maintain appropriate social distance.

Luo et al~\cite{luo_tracking_2011} demonstrate an interaction with two people and a humanoid robot head. The robot detects and tracks the face of a person in view. A pointing gesture indicates to the robot that another person is present, the robot moves its head and begins tracking the second person. 

% Additional (could be in the section above?) =================================
Lastly, robotic vision for gesture recognition was also paired with other sensor modalities to improve interaction and collaborative processes. Sensors that improve the robot perception of the interaction include speech recognition~\cite{burger_two-handed_2012, fujii_gesture_2014, vysocky_interaction_2019, yuan_development_2018, du_online_2018, maurtua_natural_2017}, surface electromyographic (sEMG) sensor (the Myo gesture control arm band)~\cite{gao_hand_2020}, Leap Motion sensor~\cite{kalidolda_towards_2018}, IMU~\cite{du_online_2018}, and wearable sensors such as a camera attached to a persons wrist to detect hand gestures are used to control a wheelchair robot~\cite{yang_novel_2018} and a dual arm robot~\cite{chen_wristcam_2019}. Other modalities provide feedback to the human, including speech response~\cite{kahlouche_human_2019,mazhar_real-time_2019, avioz-sarig_robotic_2020}, LED's that change colour in response to commands~\cite{milligan_selecting_2011, alonso-mora_human_2014}, and a display to provide decision support for operators~\cite{lambrecht_spatial_2012, sriram_mobile_2019, lalejini_evaluation_2015}, such as robot state information~\cite{chen_human-following_2019}, 

% Other sensors improved the robots actions e.g. laser~\cite{yuan_development_2017, miller_self-driving_2019}, tactile~\cite{ikai_robot_2016}.

==> ExtraFiles/scratchpad_additional_includes.tex <==

Rosenberger et al~\cite{rosenberger_object-independent_2020} safely grasp objects (e.g. banana, lemon, tin of tuna) from a human hand by first segmenting out human pixels from potential grasp locations using a Franka Panda arm.

Rosenberger et al~\cite{rosenberger_object-independent_2020} use a YOLOv3~\cite{} network for object detection, a fine tuned ResNet50~\cite{} network to segment a human hand from grasping locations on an object, and GG-CNN~\cite{} to to detect grasp locations of the segmented object. 

The EgoHands dataset~\cite{bambach_lending_2015} (15,000 images of hands) was used to train a hand detector~\cite{rosenberger_object-independent_2020}.

Pre-trained YOLOv3 to detect objects, RefineNet originally proposed by Lin [22], which was trained on the portion of the PASCAL dataset that belong to the class “Person” to detect person, hand segmentation network (per-pixel, hand or not, ResNet50 trained on custom dataset, GG-CNN to detect grasp pose, visual servoing for moving to object~\cite{rosenberger_object-independent_2020}

Kollmitz replaced by vasquez (was a duplicate paper)
Kollmitz et al\cite{kollmitz_deep_2019} classify the class label, 3D position and velocity of a person using a walking aid using a ResNet-50~\cite{he_deep_2016} and a hidden markov model (HMM). The region of interested was first extracted by the faster-RCNN, and the classifier network was pre-trained on ImageNet data and fine tuned with a custom dataset.

Hand waving has also been used to select a specific unmanned aerial vehicle from a team~\cite{monajjemi_hri_2013}. For instance, multiple unmanned aerial vehicles could detect a persons face direction, followed by robot selection when the person waves to a robot they are looking at directly. Deselection then occurs by waving with the opposite hand. The selected robots then respond to a command (e.g both hands waving down to land) ~\cite{monajjemi_hri_2013}.

Need to see if any other papers use these methods:
optic flow for hand wave detection~\cite{monajjemi_hri_2013},

 by creating a map using parallel tracking and mapping (PTAM)~\cite{monajjemi_hri_2013}
 
Almonfrey et al~\cite{almonfrey_flexible_2018} developed a vision network using four static cameras to create an intelligent work space, where a mobile robot can identify and avoid people.

Almonfrey et al~\cite{almonfrey_flexible_2018} use a vision network (4 static RGB cameras) to create an intelligent work space, where a Pioneer robot can localise itself, and follow or avoid people. 

Almonfrey et al~\cite{almonfrey_flexible_2018} train a person detectors using the INRIA dataset~\cite{dalal_histograms_2005}, containing over 1800 annotated human images.

Almonfrey et al~\cite{almonfrey_flexible_2018} compare their human detection method using a network of cameras to other methods to show they have a lower miss rate (fraction of total humans not identified), than other methods.

Gao et al~\cite{gao_user_2020} use a Gaussian mixture model to predict the motion of a human in an assisted dressing task~\cite{gao_user_2020}

From a study with 31 people in a robot assistive dressing experiment~\cite{gao_user_2020}, users were most comfortable with a method that combined a motion model, vision, and force feedback (compared to vision or force only modalities). Some users were happy to have a robot assisting them dressing.

For assistive dressing, combining a motion model, vision, and force feedback improved the reachability of a Baxter robot~\cite{gao_user_2020}. 

Mobile robot have been summoned by waving, and directed to a specific location by pointing~\cite{kahlouche_human_2019}.

Kahlouche et al~\cite{kahlouche_human_2019} fuse multiple classification methods (SVM, decision tree, and a MLP) using a voting process from an ensemble of classifiers.

TODO: replace with Vasquez:
Kollmitz et al found that RGB data performed better than DepthJet (colour-encoded depth image), and found that a VGG-CNN-M~\cite{chatfield_return_2014} provided a trade off between classification accuracy and processing speed (compared to ResNet-50~\cite{he_deep_2016} and GoogLeNet~\cite{szegedy_going_2015}) when classifying people with walking aids.


==> ExtraFiles/scratchpad_brendan.tex <==

% =============================================================================
Cameras used in gesture recognition
% =============================================================================
monocular
rgb-d
kinect



% =============================================================================
% =============================================================================
DATASETS for GESTURE RECOGNITION:
% =============================================================================
~\cite{chen_integrated_2010,martin_estimation_2010,droeschel_towards_2011,park_real-time_2011,pereira_human-robot_2013,tao_multilayer_2013,fujii_gesture_2014,xu_online_2014,canal_gesture_2015, cicirelli_kinect-based_2015, gao_humanoid_2015, potdar_learning_2016, arenas_deep_2017, ghandour_human_2017, meghdari_real-time_2017, song_towards_2017, yang_novel_2018, chen_wristcam_2019, lima_real-time_2019, kahlouche_human_2019, xu_skeleton_2020, waskito_wheeled_2020}
Required datasets:
Each gesture contains 1,000 data, with a total of 6,000 data~\cite{chen_integrated_2010}

"training set of 19 persons
including 1,710 samples."~\cite{martin_estimation_2010}

2004 pointing gestures are captured for the first stage HMM and 1656 and 348 pointing gestures are used for training and testing, respectively.~\cite{park_real-time_2011}

Custom database of gestures for matching~\cite{pereira_human-robot_2013}

We respectively recorded 10 sets of data from three experimenters for training and testing~\cite{tao_multilayer_2013}

A number of example data for each gesture were used for training of HMM~\cite{fujii_gesture_2014}

Custom dynamic gesture database~\cite{xu_online_2014}

"2082 gesture
frames and 61 gestures, 27 of them being static gestures and
the other 34 dynamic gestures."~\cite{canal_gesture_2015}

10 gestures performed by 10 different people~\cite{cicirelli_kinect-based_2015}

Training data for KNN classification, about 30 per gesture (6 gestures)~\cite{gao_humanoid_2015}

5 gestures from 2 humans, unknown how much data~\cite{potdar_learning_2016}

600 images single background + 1400 images different background~\cite{arenas_deep_2017}

"The training data is collected from four
people with different heights [152-187] cm. Each person is asked
to do 112 gestures with distances [1.7, 4] m from the Kinect, with
deviation angle [-40, 40]. Thus the total training set is 448."~\cite{ghandour_human_2017}

"10 persons, 6 males and 4 females Kinect data output was captured at least for 3 seconds
with 30 frame per second rate for each facial expression with
different head orientation. Though, each person has a dataset
that each frame of data is an array with 17 members."~\cite{meghdari_real-time_2017}

10,000 training images and 3,500 testing images, all the images are 96*96 gray level images. 5 gestures~\cite{song_towards_2017}

Custom: data collected from 5 subjects1000 gestures. Dynamic time warping algorithm for gesture classification? DTW~\cite{yang_novel_2018}

Dataset collected (For kNN?)  1350 gestures (135 videos × 10 gestures/video. 15 subjects of 7 females and 8 males. Their ages ranged from 20 to 65 years~\cite{chen_wristcam_2019}

160,000 samples from 20 individuals (15 men and 5 women). Individuals per- formed the predefined hand poses: open and closed hand. ~\cite{lima_real-time_2019}

 It was collected from 30 different people performing 33 manual gestures once. We additionally collected customized data where one person performed the same 33 gestures ten times.~\cite{kalidolda_towards_2018}

datasets used is 1000 images for each hand gesture and the number of validation data is 100 images for each hand gesture.~\cite{waskito_wheeled_2020}

Custom: OpenNI used to collect pose dataset dataset contains six interactive activitivities (4 static, 2 dynamic)~\cite{kahlouche_human_2019}


2500 gesture images are created which includes 300 images for each of ”1”- ”5” gestures, 200 images for each of ”6”-”10” gestures. There are 1200 gesture images in the test set including 120 images for each of ”1”-”10” gestures.~\cite{xu_skeleton_2020}


Trained hmm model from participant actions.~\cite{droeschel_towards_2011}


Trained in previous work:
previous work~\cite{couture-beil_selecting_2010}
Training outlined in previous work~\cite{saleh_nonverbal_2015}
Training occurs, unclear as to the database, previous work in [3]~\cite{ehlers_human-robot_2016}
previous work~\cite{maurtua_natural_2017}
Trained in previous work~\cite{martin_real-time_2019}
Unknown, possibly custom~\cite{gao_hand_2020}

Provided dataset online:

We named our dataset OpenSign~\cite{mazhar_real-time_2019} 

Available datasets:

"Cohn-Kanade
Facial Expression Database [6] and MMI Face Database [7]"~\cite{sosnowski_mirror_2010}

faceAPI, a real-time face tracking toolkit from Seeing Machines, The Inter-ACT corpus used for data, SVM smile detector~\cite{castellano_context-sensitive_2014}


FERET (Phillips et al., 1998) face database is selected for the establishment of gender identification, CK+ (Lucey et al., 2010) facial expression database is selected for the establishment of facial expression recognition~\cite{ke_vision_2016}

WIDER FACE dataset + Kaggle facial expres- sion recognition challenge dataset~\cite{li_inferring_2019}

the AffectNet Database contains approx- imately 450,000 + Cohn-Kanade (CK+) dataset includes 123 subjects and 593 image sequences. ~\cite{li_cnn_2019}






% Gesture recognition is particularly useful in loud environments such as industrial settings~\cite{}, or when the vision sensor can be used for additional components of the robots sensing ability such as object detection~\cite{}, where other human sensing modalities require an additional sensing module, such as to detect speech).


% Robots can be controlled with gestures, where a human operator must learn how to interact with the robot, or in the case that the human is a user, and the robot must learn how to interact with the human. Tasks that require gesture recognition can have a low level of autonomy where discrete gestures trigger an action from a set of pre-defined behaviours~\cite{fujii_gesture_2014}, though can also be used to input higher level human intuition, for example take the left path for an otherwise autonomous mobile robot~\cite{lalejini_evaluation_2015}. Gesture recognition can also be used to control part of the system, for example a robot arm can mimic human joint positions and hand gestures can be used to open and close a gripper~\cite{lima_real-time_2019, martin_real-time_2019}. Head recognition~\cite{saleh_nonverbal_2015} and facial expression recognition~\cite{li_cnn_2019} are examples of the robot learning the behaviours that a human performs naturally, and allow the robot to engage with the human without the human explicitly learning how to interact with the robot. We will now discuss some of the uses of gesture recognition in the three identified configurations (hand, body, and head).

% Gesture recognition has become more prevalent in robotics applications due to cheap RGB-D sensors, such as the Microsoft Kinect, and the accompanying off-the-shelf software development kits (SDK's)~\cite{}. The MS Kinect  was the most used sensor for HRI found in our search (107 papers used the MS Kinect, where RGB-D sensors overall had 127, 

% Off-the-shelf algorithms were found in more than half of the papers included in our search, including SDK's, OpenNI (open natural interaction), OpenNITE, OpenCV (open computer vision), pre-trained neural networks YOLO, OpenPose.  Off-the-shelf gesture recognition examples:



\begin{enumerate}
    \item What are the most common forms and domain areas of robotic vision in HRC/I? 
    \item What is the current state-of-the-art applications of robotic vision for HRC/I? 
    \item What is the functional impact of robotic vision in HRC/I?
    \item What are the upcoming challenges for robotic vision in HRC/I?
\end{enumerate}

The following section will provide a brief breakdown of each of the main application areas that require robotic vision, including the purpose, intended use, current level of performance, and detailed examples of its propose use in action. 

action recognition:


Gesture recognition:

purpose: to interact with a robot with unique actions from the hand, body, or face.
Intended use: For control - of a mobile or manipulator robot, or to provide a service to the human as user
current level of performance: 
detailed examples.


robot movement in human spaces:


handovers and collaborative actions:

social communication:




\technique list:

\textbf{Off the shelf}:
For practitioners looking to integrate robotic vision into their HRC/I project, off the shelf techniques are becoming more common and more powerful. 

can be used with low cost sensors like the MS Kinect~\ref{}, or with any RGB camera with . 

Available software libraries include:
OpenNI (Open Natural Interaction), which is used in this
paper, NITE Primesense, libfreenect, CL NUI, Microsoft
Kinect SDK and Evoluce SDK.

OpenFace

OpenCV~\ref{} is library that  commonly used as an interface with such as:

Viola-Jones~\cite{}, HAAR features, cascades, with adaBoosting for face detection, examples include OpenCV.

Pre-trained neural networks: OpenPose

Segmentation 

HOG features

SURF and SIFT

Other commonly used methods: SVM's, kNN

Dynamic Time Warping.

 SVM, kNN


Deep neural networks: CNN's, LSTM's, GAN's,

Non-vision techniques? (motion tracking) Kalman filter, particle filter, GMM,




% =============================================================
% =============================================================
% =============================================================



Task	
Grasp Assistant 	Moving something to a human (by grasping)
Gesture Control	Drones, anything that is controlled through gesture
Mobility Assistant	Moving a human
Social Mobile	Any mobile platform with the primary task of mobility (following, avoiding, approaching human). Only robots that don't interact at a higher social level
Social Gesture	Mobile robots that are a bit more sophisticated than just mobile. Exercise robots, robots that engage physically
Social Emotive	Robots that converse with people with face gesture recognition
Other	e.g. infrustructure inspection, drip stand robot (add to to this list, then can consider new classes)
	
Robot	
Mobile	
Fixed Manipulator	
Mobile Manipulator	
Drone	
Social	Mobile social robot should be classified by primary task (mobile or social)
	
Domain	
Field	Outside applications
Industrial	Including manufacturing and warehouse
Domestic	Home, can include healthcare (targeted at home)
Urban	Shopping centre, school, restaurant, can include healthcare (hospital)


	
Robotic Vision	
Gaze estimation	Includes eye tracking and head pose tracking
Human pose tracking	No classification, just is there a person, and where
Human pose recognition	Includes disability classification and pose estimation / identification / classification
Hand tracking	No classification, just is there a hand, and where
Hand gesture recognition	Includes gesture classification
Face tracking	Includes face detection and head tracking
Face recognition	Detecting gender, or specific person
Face gesture recognition	Includes emotion recognition
Other	Human not present in vision part (consider excluding paper?)

-

List of robots commonly used, a list of tasks commonly performed
HRC robots:
\begin{itemize}
    \item Robot arms (Jaco, Kuka) 
    \item Humanoids (Nao, Pepper)
    \item Mobile bases (Pioneer)
    \item Mobile base with arms (PR2, robot arm mounted to wheelchair)
    \item Social (Humanoids, FurHat)
    \item Aerial and underwater
\end{itemize}

HRC tasks:
\begin{itemize}
    \item Reaching/manipulation assistance
    \item Person following
    \item Instruction providing
    \item 
\end{itemize}

How is vision used
HRC vision sensor types:
\begin{itemize}
    \item RGB
    \item Depth
    \item RGB+D e.g. Kinect (RBG + D, or TOF)
    \item 
\end{itemize}

HRC vision algorithms:
\begin{itemize}
    \item 
\end{itemize}

Gesture recognition

With or without robot (robot response/action is not considered)

High speed single camera techniques are emerging. ~\cite{katsuki_high_speed_2015} use a single high speed camera predict the configuration of human hand. This could enhance efficiency in production processes by cooperating with humans on tasks swiftly.

~\cite{xia_vision-based_2019} binocular vision for hand gesture segmentation and extraction. \textbf{No robot} 

~\cite{gori_multitype_2016} develops an algorithm for activity recognition from multiple people in a robots view (RGBD). Computation is performed in real time, though currently limited to two people. Autonomous mobile robot with a MS Kinect is used to collect data from a natural environment with students.

~\cite{jevtic_comparison_2015}assesses three control modalities including push, following, and pointing to guide a mobile platform to specific rooms in domestic setting. For service robot applications where the robot is guided to a location by a human. Uses off the shelf person detection and skeleton joint tracking (Microsoft Kinect SDK). Concludes that pointing is worse (time taken, accuracy, stress on the human) than pushing, but there are applications where pushing might not be possible. 

~\cite{shukla_probabilistic_2015} looks at finger pointing, in particular creates a probabilistic method for estimating the pose of a pointing finger (or pointing tool) to identify a target object, such that a human can point to an object and a robot can pick it up. Uses RBGD, and a grasping robot arm (couldn't see any details about the robot). Pointing is determined independently of body pose, and is invariant to size and scale of pointing gesture. In a followup work in simulation and on a real platform, ~\citep{shukla_proactive_2017} demonstrates the human can point to an object, signal "give me", and handover of the object. This is demonstrated the task of assembling furniture, where the robot hands the human the legs to a table. 


Reverse gesture recognition? Robot provides the gesture ~\cite{admoni_modeling_2016}


% ExClude papers that investigate the social outcomes? ~\cite{mead_proxemics_2015} investigate the distance of a mobile robot from a human providing instructions, either by speech or by pointing. This study looks at the experience of the human subject (robot competence, anthropomorphism, engagement, likability, and technology adoption), as well as the performance of the speech and gesture recognition over at different distances from the human (speech and gesture recognition degrade with distance). The robot is mobile with a humanoid upper torso. Might be a better fit in an another place (proxemics is the main priority).

==> ExtraFiles/scratchpad_includes.tex <==
% ==================================================

===================================================================================================
\subsubsection{Social}
===================================================================================================

Robots:
little humanoid~\cite{igorevich_behavioral_2011, indrajit_development_2013, lu_research_2020}. Zeno humanoid~\cite{torres_implementation_2012}, 4
Nao~\cite{yang_study_2013, taheri_social_2014, zhu_robust_2017, gong_research_2018} 4
Pepper~\cite{bilac_gaze_2017, sorostinean_activity_2018, cazzato_real-time_2019, jarosz_detecting_2019, augello_towards_2020, lee_visual_2020} 6

Other: 5
humanoid robot receptionist~\cite{li_visual_2015}
Wheeled base, humanoid torso ~\cite{phong_vietnamese_2020}
ROMAN humanoid torso~\cite{saleh_nonverbal_2015}
Harley humanoid~\cite{li_cnn_2019}
iCub~\cite{boucher_i_2012}

5
icat~\cite{castellano_context-sensitive_2014} (with arms),

head robots:  
Eddie~\cite{sosnowski_mirror_2010}, Reeti~\cite{masmoudi_expressive_2011}, and Alice~\cite{meghdari_real-time_2017, taheri_social_2014} robot. 

HSR~\cite{lee_visual_2020}, mobile with manipulator
irobot create~\cite{zhang_optimal_2016}
Kompaï mobile Robot~\cite{vaufreydaz_starting_2016}
Pioneer 3-DX~\cite{chien_navigating_2019}
mobile robot~\cite{li_inferring_2019}
ARIO mobile robot~\cite{tseng_multi-human_2014}
===================================================================================================

Facial expressions were used to control an anthropomorphic social robot head by mimicking human expressions, such as the  Eddie~\cite{sosnowski_mirror_2010}, Reeti~\cite{masmoudi_expressive_2011}, and Alice~\cite{taheri_social_2014, meghdari_real-time_2017} robot. Alice with body~\cite{taheri_social_2014}.


Humanoid robots were required to copy human joint positions~\cite{igorevich_behavioral_2011, csapo_multimodal_2012, torres_implementation_2012, indrajit_development_2013, yang_study_2013, taheri_social_2014, zhu_robust_2017, augello_towards_2020, lu_research_2020}, including head position~\cite{cazzato_real-time_2019}. speaking and face detection for conversation, teleop nao robot through kinect~\cite{csapo_multimodal_2012}. NAO and alice with body robot mimic human pose using kinect. Also haptic device as a control option. Alice can smile, robots can help teach colours.NAO pointing and changing eye colour for children to identify~\cite{taheri_social_2014}. On pepper~\cite{augello_towards_2020}.



Robot uses vision to determine social configurations of people and approaches accordingly, groups of two people, ARIO robot~\cite{tseng_multi-human_2014}



Robot reaches for object human asks for and looks at, iCub + speech~\cite{boucher_i_2012}

Robot bartender James= icat with arms, senses people with vision, interacts and takes orders for drinks, with multiple people.~\cite{foster_two_2012}

Small UAV hovers above the hand of person wearing a blue glove, and can be passed from one person to another~\cite{miyoshi_above_2014}. Uses 2 cameras

Nao robot detects user from vision and sound, and responds accordingly~\cite{cech_active-speaker_2015}.

humanoid robot receptionist conversation with vision, determines the direction of attention of human.~\cite{li_visual_2015}. humanoid robot receptionist

Face emotion detection and response robot head. e.g. if male sad, robot shows surprise then sad, if female sad, robot shows interest then guilt~\cite{ke_vision_2016}.

Molleret et al~\cite{mollaret_multi-modal_2016} use a PR2 robot to approach, and interact with a person when it detects intention for interaction.

detect if robot should engage person~\cite{vaufreydaz_starting_2016}. Kompaï Robot, social robot with head shape, vision + laser + ultrasound + infrared + touchscreen

Gaze detection by mobile robots - uses vicon motion capture~\cite{zhang_optimal_2016}, irobot create

Learning natural social communication through gaze and speech breaks with pepper robot~\cite{bilac_gaze_2017}

Detect person face with nao robot with camera, wave when person waves detected with wearable imu.~\cite{gong_research_2018}.

This is in action rec as well~\cite{sorostinean_activity_2018}. pepper robot detects activity and responds with questions and change in state.CNN + LSTM using skeleton data (SDK)

Pepper mimic head position~\cite{cazzato_real-time_2019}.

Person and gender recognition (discern staff, patient, stranger), obstacle avoidance, and person following~\cite{chien_navigating_2019}. Pioneer 3-DX, plus stand and kinect at the base rgb on top Chien et al perform gender classification and person identification to follow a person~\cite{chien_navigating_2019}. The robot also has a sonar sensor for obstacle avoidance.

pepper robot conducts interview, persons gaze determines actions (peppers speech)~\cite{jarosz_detecting_2019}

mobile robot approaches person if it should. two people. (determined by body pose and several factors including facial recognition (happy, sad, angry etc..)~\cite{li_inferring_2019}

emotion detection triggers pre-defined robot response. Harley humanoid~\cite{li_cnn_2019}

Socialise with people in restaurant (point to seating locations, repeat bar orders), Fetch object and deliver (requires relocation of human)Pepper, and HSR~\cite{lee_visual_2020}.

humand mimics human~\cite{lu_research_2020}

reception robot, conversation, uses vision to detect person is there~\cite{phong_vietnamese_2020}. Wheeled base, humanoid torso


Gestures such as nodding or shaking of the head were used in social interactivity, including to evaluate human engagement~\cite{saleh_nonverbal_2015}. For instance, facial expression and gaze detection were used to determine children engagement in an educational program~\cite{castellano_context-sensitive_2014}. Facial expressions and body pose were used to evaluate if a mobile robot should approach a human~\cite{li_inferring_2019}.


A mobile social robot determines the appropriate time to approach a human after inferring user intent through body gestures and facial expressions~\cite{li_inferring_2019}. For these demonstrations there is often more than one human in the robot field of view, and the robot must at all times maintain appropriate social distance.

\subsubsubsection{Social techniques}
% ==================================================

Joint positions extracted from RGB-D sensor~\cite{igorevich_behavioral_2011, torres_implementation_2012, indrajit_development_2013, yang_study_2013, taheri_social_2014, tseng_multi-human_2014, mollaret_multi-modal_2016, meghdari_real-time_2017, augello_towards_2020, lu_research_2020}

% ==================================================

 iCub gaze controller~\cite{boucher_i_2012}

ms sdk + viola jones~\cite{csapo_multimodal_2012}

colour segmentation + blob detection and tracking ~\cite{foster_two_2012}

two cameras and colour segmentation for little uav~\cite{miyoshi_above_2014}.

moving average and butterworth filter for joints from kinect~\cite{taheri_social_2014}.

approaches people after detecting TODO~\cite{tseng_multi-human_2014}

Face Detector [27], Identity Recognition (identity, age, and gender) [28], [29], Face Tracking [30], Sound Recognition [25], Sound Localization and AV Fusion (described in this paper).~\cite{cech_active-speaker_2015}.

viola-jones haar classifier and cascades, DMP (Direction-Magnitude Pattern) features, SVM. Head gestures from direction and magnitude pattern of depth pixels were classified with a SVM~\cite{saleh_nonverbal_2015}.

Opencv haar features viola-jones and cascades, trained for eye, nose, mouth. Gabor filters, PCA, and SVM~\cite{ke_vision_2016}

Random forests for real time 3D face analysis for line of sight OpenNi for body pose. Detects desire to interact with head/shoulder pose, speech. Voice Activity Detection (VAD). particle swarm optimization inspired tracker, tracking and voice are fused for HMM.~\cite{mollaret_multi-modal_2016}

Minimum Redundancy Maximum Relevance (MRMR)~\cite{vaufreydaz_starting_2016}. 29 interactions with the robot,made by 15 different participants, 5 classes for interact, leave interact etc.. 158000 frames

ROS face recognition package - Viola-jones but using depth to remove false positives based on realistic size of face.~\cite{zhang_optimal_2016}

Train filled pause detector (speech), when detected use peppers gaze detector for 1.5s, make a decision whos turn to speak~\cite{bilac_gaze_2017}

MS SDK + Neural network~\cite{meghdari_real-time_2017}

Velocity (MV) Algorithm and RVM, robust regress-based refining. I think they use an sdk~\cite{zhu_robust_2017}

OpenCV, no details of method used for face detection~\cite{gui_teaching_2018}.

This is in action rec as well~\cite{sorostinean_activity_2018}. pepper robot detects activity and responds with questions and change in state.CNN + LSTM using skeleton data (SDK)

ResNet-10 SSD + OpenFace, pre-trained networks~\cite{cazzato_real-time_2019}.

"Fuzzy combination of depth and sonar. penCV’s
OpenCV’s LPBH (Local Binary Patterns Histogram) face recognizer method"~\cite{chien_navigating_2019}

custom gaze detection  - detection face, detect landmarks on face, eye regions, head pose, pupil centre~\cite{jarosz_detecting_2019}

SSD for face detection, NN- facial recognition model. random forest regression, ~\cite{li_inferring_2019}

HAAr features for detecting face region, CNN and LSTM (custom network, search through parameters)~\cite{li_cnn_2019}

OpenNI~\cite{augello_towards_2020}

From extracted features, classification of gestures was performed with traditional machine learning methods such support vector machines (SVM)~\cite{saleh_nonverbal_2015, ke_vision_2016}. SVM's facial expressions~\cite{sosnowski_mirror_2010, castellano_context-sensitive_2014, ke_vision_2016}. Head gestures from direction and magnitude pattern of depth pixels were classified with a SVM~\cite{saleh_nonverbal_2015}. Other methods use feature extractors such as Gabor filters~\cite{ke_vision_2016}. 
Neural network layers that utilise time-series (such as LSTM) are also used to classify dynamic gestures~\cite{li_cnn_2019}.


Recent works use convolutional neural networks to detect the face region ~\cite{li_inferring_2019, li_cnn_2019}. The face location can be used to then classify facial expressions~\cite{li_cnn_2019},

~\cite{lee_visual_2020}semantic slam

OpenNI~\cite{lu_research_2020},

MS SDK for head pose detection~\cite{phong_vietnamese_2020}

OpenCV 2 cascade face detector, which is based on the Viola and Jones and openCV for locating facial features. Emotion classification ~\cite{masmoudi_expressive_2011}

Deep neural networks have been adopted for gesture classification in recent years. The most common usage was convolutional neural networks (CNN's), classifying gestures directly from pixels. Alternatives perform classification from the extracted skeletal information~\cite{}. architectures and use pre-trained models that are then fine tuned on task specific data~\cite{mazhar_real-time_2019, waskito_wheeled_2020}, or trained with a custom dataset~\cite{gao_hand_2020}. Examples of papers that investigate their own network architecture include~\cite{li_cnn_2019}. Li et al~\cite{li_inferring_2019} TODO: SSD for face detection + other things. Li et al~\cite{li_cnn_2019} use a CNN with LSTM to detect facial expression changes.

\subsubsubection{Cameras Used for Social Classification and Communication:}

From the 41 papers identified that required the robot to communicate with a human in an social interaction, the most common camera type was the RGB-D sensor ($n=24$), followed by monocular RGB cameras ($n=15$). In the 24 papers that used an RGB-D camera, 23 used the Microsoft Kinect. Two papers ($n=2$) used a stereo camera.

\subsubsubsection{Datasets/Models:} 

Papers that used datasets from external sources were most commonly used for facial expression recognition~\cite{sosnowski_mirror_2010, castellano_context-sensitive_2014, ke_vision_2016, li_inferring_2019, li_cnn_2019}. The Cohn-Kanade dataset~\cite{kanade_comprehensive_2000} and its extended form (CK+)~\cite{lucey_extended_2010} was used to train facial expression models~\cite{sosnowski_mirror_2010, ke_vision_2016, li_cnn_2019}. Other datasets include FERET, AffectNet, MMI Face Database, and the Inter-ACT corpus. Several papers built on previous work for gesture recognition models (the details of datasets used in training were not provided)~\cite{saleh_nonverbal_2015}. 

the AffectNet Database contains approx- imately 450,000 + Cohn-Kanade (CK+) dataset includes 123 subjects and 593 image sequences. ~\cite{li_cnn_2019}

Datasets that use video~\cite{meghdari_real-time_2017}
"10 persons, 6 males and 4 females Kinect data output was captured at least for 3 seconds with 30 frame per second rate for each facial expression with different head orientation. Though, each person has a dataset that each frame of data is an array with 17 members."~\cite{meghdari_real-time_2017}

Trained on: Aberdeen Facial Database, GUFD Facial Database, Utrecht ECVP Facial Database + images of laboratory personel using openCV’s LPBH~\cite{chien_navigating_2019}.

WIDER FACE dataset + Kaggle facial expres- sion recognition challenge dataset~\cite{li_inferring_2019}




===================================================================================================
\subsubsection{Learning from demonstrations}
===================================================================================================
Human demonstrates actions observed with vision, robot executes. iCub, actions include Hold, place, take~\cite{saegusa_cognitive_2011}

track hand position, and object, and action, to mirror and perform by robot. Segmentation and blog detection~\cite{saegusa_cognitive_2011}


Industrial arm programmed, and controlled with gestures, Body: lifting the foot to start programming, arm position to encode open/close gripper and position.~\cite{stipancic_programming_2012}. 6-axis FANUC robots

Kinect sdk, joint angle geometry? (not mentioned how gestures are classified)~\cite{stipancic_programming_2012}

Kinect input to update robot behaviour on a humanoid based on periodic dynamic movement primitives~\cite{petric_online_2014}Sarcos humanoid ms SDK?


Little humanoid learns behaviours from demonstration from 2 agents through kinect . ~\cite{potdar_learning_2016}, Supervised learning LSTM for learning how a human responds to another human, then transfered to the robot

Robot follows human with gaze, and follows several aspects of a watering task. Simple statemachine, not sure of the utility. Several vision components~\cite{yoo_gaze_2017} Opencv cascade haar features for face viola jones, CNN to detect objects, 


Teaching robot through gestures and speech for industrial arm~\cite{du_online_2018}. Kuka arm. interval kalman filter, improved particle filter, 


Learning from demonstrations for peg grasping task for humanoid torso with kinect ~\cite{li_learning_2018}. imNeu humanoid torso. OpenNI, Gaussian mixture model and GMM regression


kuka arm learns from demonstrations, with gesture control, and safety factors ~\cite{mazhar_real-time_2019}. OpenPose library, Inception V3 convolutional neural network is adapted and trained to detect the hand gestures + fine tuning 


===================================================================================================
\subsubsection{Handover and collaborative actions}
===================================================================================================

Robotic kitchen, uses vision to interact with disabled person~\cite{aranda_friendly_2010}

ASIMO humanoid robot follows the head pose of an operator for direction while mimicking hand position with its end effector to handover an object (a green marker) to another person~\cite{arumbakkam_multi-modal_2010}. 

Jido robot approaches a person with proxemics in mind to hand over a water bottle to a seated person  "sufficiently far from the human and yet sufficiently near to achieve hand over task" ~\cite{sisbot_synthesizing_2010}. Trajectories are synthesised based on safe and socially acceptable distances.

Industrial robot arm avoids human that has coloured markers attached, detected with stereo vision~\cite{ding_optimizing_2011}

Staubili tx90 robot arm,  multiple people with camera network, industrial arms deactivate when humans get close~\cite{nair_3d_2011}

An ABB industrial 4 actions: warn the operator, stop the robot, move back, and modifying the path ~\cite{wang_vision-guided_2013}.

Multiple kinects create a safe workspace for  Lab-Volt 5150 5 DOF manipulator arm~\cite{morato_toward_2014}. Robot stops when human close. Chassis assembly task.

Kinect sensor is used to track a persons hand in an screwing task with a Kuka arm~\cite{cherubini_unified_2015}. Force sensor is also used.

ABB Industrial arm TCP goes to location of human hand (mimic movement)~\cite{christiernin_interacting_2016}


A human points to an object (See gesture recognition). Once picked up, the hand over process relies on the tactile sensors on the finger tips to know when shear has occurred (the object is in the palm)~\cite{ikai_robot_2016}.

Cooperative folding of a sheet, human hand is detected against fabric corner, robot picks up the opposite corner to folder.~\cite{koustoumpardis_human_2016}. Adept Cobra s800

Safe workspace, robot arm plans to avoid human~\cite{moreno_path_2016}.


Soft robot follows humans back using kinect and ultrasonic sensor for washing robot~\cite{dometios_real-time_2017}.5 DOF Katana arm by Neuronics

FUM SCARA style robot arm, safe workspace, stops if human detected~\cite{shariatee_safe_2017}

Kuka arm stops when human enters shared workspace~\cite{araiza-lllan_dynamic_2018}

Robot arm moves as hand moves in 3D. Can also grasp when two hands out in front. UR10 with hand gripper~\cite{bolano_towards_2018}


Shared workspace with a UR3 arm~\cite{bothe_effective_2018}

Direct control of unknown robotic arm~\cite{hong_interactive_2018}, no gripper.

Safe workspace, detection and avoidance Kawasaky RS005LA~\cite{pasinetti_development_2018}.

Person detection, then gesture from wearable imu, Kuka arm~\cite{haghighi_integration_2019}

Cameras detect surgeon gaze to determine what instrument a UR5 robot should fetch during an operation~\cite{kogkas_free-view_2019}

Robot Fanuc LR Mate 200iD/7L, tracks human hand and changes path if it gets too close~\cite{landi_prediction_2019}

Handover with robot arm and hand tracking using UR3\cite{scimmi_experimental_2019}. Human to robot handover.

Robot picks up show and brings it to human foot~\cite{valle_personalized_2019}. Speech is also used for the state machine. WAM robot arm. Dressing assistant. Robot to human handover.

dual arm panda robot. Velocity at end-effector is reduced when human detected~\cite{zardykhan_collision_2019}. safe workspace

Feeding assistance robot operated with eye tracking glasses~\cite{arai_service_2020}. Unknown robot arm. Eye glasses use near a infrared camera, robot arm has a camera attached, the person can see the camera feed through a hmd.

Safe workspace with kuka arm, also uses touch~\cite{bingol_practical_2020}. 

robot arm avoids collision with human, ~\cite{chan_collision-free_2020}, HIWIN industrial arm

shared workspace, human detection and avoidance~\cite{ferraguti_safety_2020}, 6-DoF Puma 260 robot.

Safe workspace~\cite{liu_dynamic_2020}robot avoids human in safe workspace. ABB industrial arm 

Collision avoidance, safeworkspace, ~\cite{mronga_constraint-based_2020}. Kuka arm


safe workspace with baxter and human~\cite{tarbouriech_bi-objective_2020}

Robot adjusts work height based on human pose~\cite{van_den_broek_ergonomic_2020}. Sawyer robot arm

~\cite{zhang_human_2020}. Collaborative manipulation task, kinect + IMU's to predict human pose. Franka panda arm

Handover robot to human, using force sensors~\cite{bdiwi_handing-over_2013}.Staubili RX90 robot with a JR3 multi-axis force/torque sensor


Dual arm Baxter robot is used to assist with dressing, where the robot helps people put on a jacket with sleeves~\cite{gao_user_2020}.


Human monitoring in safe manufacturing setting (cellular manufacturing)~\cite{tan_safety_2010}. Human wears colour markers on their helmet, and a light curtain indicates to the human the extents of the safe workspace.

Human to robot handover, human is segmented out of the image so the object can be safely grasped, Panda arm, grasping various objects, e.g. banana, lemon, tin of tuna,  ~\cite{rosenberger_object-independent_2020}.


% ==================================================
% ==================================================
% Techniques for handover
% ==================================================
% ==================================================
Unknown~\cite{aranda_friendly_2010}. Consider removing, design paper

Viola-jones for face detecdtion, particle filter for head tracking, joint positions from depth camera~\cite{arumbakkam_multi-modal_2010}.

Unclear vision technique~\cite{sisbot_synthesizing_2010}.

coloured markers tracked with stereo cameras~\cite{ding_optimizing_2011}

segmentation, detection, occulsion checking, tracking~\cite{nair_3d_2011}

Two kinect cameras detect the operator with kinect SDK, a 3D model of the robot is used determine the location of the robot.~\cite{wang_vision-guided_2013}


Multiple kinects provide skeleton sdk, motion model of person, particle filter, and Kalman filter~\cite{morato_toward_2014}

Kinect sdk to get hand position, force sensor is also used in the collaboration. ~\cite{cherubini_unified_2015}

MS sdk is used to get human joints, ~\cite{christiernin_interacting_2016}

largest skin-colored area other than the face area. In addition, the palm’s centroid is obtained ( stereo vision). Tactile sensor knowns when shear force is greater than a threshold (releases object)~\cite{ikai_robot_2016}

Skeleton tracking with OpenNI libraray (using opencv), moving average filter to reduce errors, rgb-d visual servoing, and a neural network force feedback controller~\cite{koustoumpardis_human_2016}.

Kinect sdk used to get joint positions, inverse kinematics used to plan a trajectory that avoids the human~\cite{moreno_path_2016}

uses depth camera for surface shape of human back~\cite{dometios_real-time_2017}

distance threshold, binary image, morphology, sobel edge detection~\cite{shariatee_safe_2017}.

OpenNI to get skeleton info~\cite{araiza-lllan_dynamic_2018}.

Point cloud obtained from depth sensor, hands detected a certain distance out in front. Velocity of TCP controlled with the position of the users hand using a UR10 robot arm. When the user places two hands out in front the gripper closes, for picking up ball task~\cite{bolano_towards_2018}.

Shared workspace using Microsoft SDK for skeleton extraction~\cite{bothe_effective_2018}.

Microsoft SDK for joint positions for direct control. Also uses Savitzky-Golay
smoothing filter~\cite{hong_interactive_2018}.

HOG + svm for detection and avoidance~\cite{pasinetti_development_2018}.

Unknown detection, imu for gesture~\cite{haghighi_integration_2019}.

Gaze and head pose detection (eye tracking with proprietary method)~\cite{kogkas_free-view_2019}

Robot tracks human hand using the Microsoft SDK, and has a motion model of the person (using semi adaptable neural network to model the human hand position with minimium jerk), predicting collision with the robot path~\cite{landi_prediction_2019}.

Microsoft SDK for skeleton (two kinects)~\cite{scimmi_experimental_2019}.

Ms SDK for skeleton~\cite{valle_personalized_2019}.

OpenPose for skeleton, two components of a detection system: Impulse Orb (collision detection), and end-effector trajectory planning ~\cite{zardykhan_collision_2019}

Vison CNN trained in previous work~\cite{bingol_practical_2020}.

Get skeleton from rgb-d~\cite{chan_collision-free_2020}

OpenCV adaptive thresholding for pupil detection, gaze direction determined from distance from the center of the image~\cite{arai_service_2020}.

~\cite{ferraguti_safety_2020} skeletons from two rgb-d 

MS SDK for human pose~\cite{liu_dynamic_2020}.

Kinematic Continuous Colli- sion Detection Library (KCCD) (voxelise stuff in the robot path?) ~\cite{mronga_constraint-based_2020}
 
Bi-directional RRT + 3d occupancy grid, unsure how human detection is performed~\cite{tarbouriech_bi-objective_2020}
 
openPose (with ROS)~\cite{van_den_broek_ergonomic_2020}.
 
~\cite{zhang_human_2020} skeleton from kinect, fused with IMU data to track pose.

Visual servoing, detect and segment objects, handover with force sensors~\cite{bdiwi_handing-over_2013}.
 
OpenNI ROS to get skeleton information. GMM motion model of human joints, with vision and force feedback~\cite{gao_user_2020}. 

Colour segmentation with two cameras to determine where the human is~\cite{tan_safety_2010}.

Pre-trained YOLOv3 to detect objects, RefineNet originally proposed by Lin [22], which was trained on the portion of the PASCAL dataset that belong to the class “Person” to detect person, hand segmentation network (per-pixel, hand or not, ResNet50 trained on custom dataset, GG-CNN to detect grasp pose, visual servoing for moving to object~\cite{rosenberger_object-independent_2020}

===================================================================================================
\subsubsection{Action Recognition}
===================================================================================================

Walking style prediction~\cite{kollmitz_deep_2019, chalvatzaki_learn_2019}, exercise robot~\cite{werner_evaluation_2013, gorer_autonomous_2017, avioz-sarig_robotic_2020}, home service robots~\cite{koppula_anticipating_2016} and robot arms~\cite{lee_learning_2017, wang_collision-free_2017}.  Use cases for visual detection were often actions to directly assist a human, such as with a robotic walker~\cite{chalvatzaki_learn_2019}, playing a game~\cite{efthymiou_multi-_2018}, clearing a table~\cite{lee_learning_2017}, or opening a fridge~\cite{koppula_anticipating_2016}). Additional feedback provided by the robot, such as blinking and face tracking, provided the user with a more pleasant experience~\cite{gorer_autonomous_2017, avioz-sarig_robotic_2020}.

With action recognition the robot should recognise what a human is doing to provide assistance without specific human instruction. In comparison to the other application areas, action recognition is a newer area of research (most papers are from the past few years). Accurate classification of human actions is a difficult vision problem, and requires large datasets to train time series classifiers (such as the use of Long Short Term Memory (LSTM)~\cite{HochSchm97} or Gated Rectified Unit (GRU)~\cite{cho-etal-2014-learning} blocks).

Example methods: Papers that use LSTM:~\cite{potdar_learning_2016, wang_collision-free_2017, sorostinean_activity_2018, chalvatzaki_learn_2019, li_real-time_2019}, papers that use GRU:~\cite{gui_teaching_2018}. Other methods: Hidden Markov Models (HMMs)~\cite{zhuang_learning_2016}, change of position over time (between frames)~\cite{lang_research_2020}, stacked frames (16 images) from multiple kinects fed through a CNN~\cite{efthymiou_multi-_2018}. Not really sure, something to do with segmentation~\cite{saegusa_cognitive_2011}.

==========TODO:
More details about~\cite{efthymiou_multi-_2018}, though I think they are out of scope:
For the first pipeline of our single- view action recognition system, the state-of-the-art Dense Trajecto- ries (DT) [21] features are combined with the Bag of Visual Words (BoVW) encoding framework. In each video frame, dense points are sampled and tracked through time based on a dense optical flow field. The features that are computed along each trajectory are: the Trajectory descriptor [21], Histograms of Oriented Gradients (HOG) [22], Histograms of Optical Flow (HOF) [22], and Motion Boundary Histograms (MBH) [21] computed on both axes (MBHx, MBHy). Encoding of the features using the BoVW and assignment to K=4000 clusters follows in order to form a representation of each video. Videos are classified based on their BoVW representation, using non-linear Support Vector Machines (SVMs)

===================================================================================================
\subsubsection{Robot Movement in Human Spaces}
===================================================================================================


Re-identification using audio~\cite{luo_human_2010}.


Laser for leg detection~\cite{luo_human_2010, alvarez-santos_feature_2012, pereira_human-robot_2013, weinrich_appearance-based_2013, hu_design_2014}, or shoulder detection~\cite{kobayashi_people_2010}.

Laser for obstacle avoidance~\cite{yun_robotic_2013, ali_improved_2015, yang_socially-aware_2019}.

Laser for navigation using SLAM~\cite{do_human-robot_2014, angonese_multiple_2017, yuan_development_2018, miller_self-driving_2019}. Miller et al~\cite{miller_self-driving_2019} follow a human by giving the robot position goals in its occupancy map that are a fixed offset from the tracked human

Ultra-sonic sensor for person following, where the person must hold a coloured marker~\cite{hassan_computationally_2016}. Sonar for navigation~\cite{chien_navigating_2019}.


Multi-human environment~\cite{yang_socially-aware_2019}

Pioneer:~\cite{jia_autonomous_2011, alvarez-santos_feature_2012, pereira_human-robot_2013, yun_robotic_2013, hu_design_2014, munaro_fast_2014, chen_stereovision-only_2014, ali_improved_2015, gupta_robust_2015, angonese_multiple_2017, almonfrey_flexible_2018, chien_navigating_2019}. 


Tracking should be in the techniques section
Face tracking:
~\cite{fahn_real-time_2010, cheng_multiple-robot_2013, bayram_audio-visual_2016, weber_follow_2018, yao_monocular_2017}

body tracking (using extracted skeleton:
~\cite{kahily_real-time_2016, anuradha_human_2020}

Other forms of tracking (e.g. through SURF features, or histogram analysis):
~\cite{chen_person_2012, wu_accompanist_2012,  weinrich_appearance-based_2013 } KCF


Following =============================
==========================================
Following with gestures: 7. 
Papers:

Person following using face tracking~\cite{fahn_real-time_2010}

Person following for wheelchair and museum robot, laser to get shoulder contours, then head position~\cite{kobayashi_people_2010}

Person following with mobile robot using SURF features~\cite{chen_person_2012}.

Other mobile platforms included the SCITOS G5 mobile robot~\cite{weinrich_appearance-based_2013, weber_follow_2018}. Weinrich et al~\cite{weinrich_appearance-based_2013} use lasers to detect a persons legs, and an omni-directional camera to detect, track, and re-identify a person . Weber et al use perform person following using face tracking with a monocular camera~\cite{weber_follow_2018}. 

Bayram et al~\cite{bayram_audio-visual_2016} use audio localisation to allow a robot to find a person when they are not in view. Once the robot can see the person, it performs face tracking and is able to detect multiple people. Nguyen et al~\cite{nguyen_audio-visual_2014} also localise a person that is out of view using sound, and once in view, a target person (from multiple people) is tracked when they wave.

Person following with mobile robot, openi when static, voxelisation and segmentation when moving~\cite{kahily_real-time_2016}.

Yao et al~\cite{yao_monocular_2017} use a monocular camera attached to an autonomous blimp robot to detect and track a persons face.

Medical nurse robot follows with skeleton tracking~\cite{long_kinect-based_2018}

Turtlebot detects, tracks and follows human~\cite{condes_person_2019}. Re-identifies specific target face when they go out of view.

Mecanum mobile robot follows human~\cite{luo_real-time_2019}.

Wheelchair follows person~\cite{wu_improved_2019}.

Person following with vision using target contour bands~\cite{zhang_vision-based_2019}.

Person following with vision using Kinect SDK~\cite{anuradha_human_2020}.

Person following with vision, SSD, facenet and KCF tracking~\cite{hwang_interactions_2020}

Drip stand robot follows person wearing a particular colour pattern~\cite{wu_toward_2020}.

Sound to re-identify lost person, person detection from custom dataset, person following~\cite{luo_human_2010}


Approaching =============================

Line following robot, approaches person when face detected~\cite{budiharto_indoor_2010}.

A PR2 robot approaches a person using a real-time proxemic controller~\cite{mead_probabilistic_2012}.

A mobile R2D2 robot with arms, carries a smaller mobile robot with a gripper~\cite{cheng_multiple-robot_2013}. The mother robot detects a persons face and waves. The robot can also deliver a drink based on the distance to the target persons face. Lastly, the mother robot deploys a smaller robot with a gripper to pick up small objects in its path.

Tibi robot (mobile base with anthropomorphic body and head) approaches people searching for an interaction~\cite{ferrer_robot_2013}.

Chen et al~\cite{chen_stereovision-only_2014} use a pioneer robot to detect and approach a persons face using stereo vision. 

% Avoiding =============================

Person avoiding with mobile robot, HOG features and svm~\cite{talebpour_-board_2016}.

Mobile robot detects people and adjusts velocity~\cite{vasconcelos_socially_2016}

Autonomous people avoidance, people can also use gestures to signal the preferred path of the robot.~\cite{ghandour_human_2017}

Avoid people using a social force model that allows for appropriate social distance when passing~\cite{yang_socially-aware_2019}. Laser for obstacles.

% Avoiding or following:
A vision network (4 cameras) is used to create an intelligent work space, where a mobile robot can localise within a smart space, and follow or avoid people~\cite{almonfrey_flexible_2018}


% Other ===============================

A team of iRobot create platforms navigate through an urban environment detecting human faces and reporting back to a supervisory person~\cite{do_human-robot_2014}. The robots have an omni-directional camera for person detection, and a laser that is used to navigate through the environment (using SLAM).

Multiple people are detected and used as landmarks for integration into a SLAM solution for a mobile pioneer robot following a path~\cite{angonese_multiple_2017}.

% ==============================

RHMS techniques:

% Examples ======================================================
% Face detection with Viola-Jones~\cite{budiharto_indoor_2010, lam_real-time_2011}.

A particle filter is used to track a face~\cite{fahn_real-time_2010}. Face is in the center of the screen at the beginning of the interaction, the colour spectrum of the skin and hair are determined and tracked using a particle filter.

Laser information to get the contours of the shoulder, viola-jones to get face information. Tracked with particle filter.~\cite{kobayashi_people_2010}

Images are first converted to a local binary pattern~\cite{ojala_lbp_2002} to be robust to lighting~\cite{yun_robust_2010}. 

Laser for legs, weighted features for human detection including LBP~\cite{ojala_lbp_2002}, canny edge detector~\cite{canny_computational_1986}, and histogram of gradients (HOG~\cite{dalal_histograms_2005})~\cite{alvarez-santos_feature_2012}

Laser for leg detection, face detection with viola-jones, and then SURF features to match clothing~\cite{wu_accompanist_2012}.

SURF features~\cite{bay_speeded-up_2008} are used to track a person wearing a known pattern~\cite{chen_person_2012}.

Disparity image is taken from a stereo camera, a canny edge detector is used to extract a human shape, the head is segmented using geometry, and compared to a samples from a model image using Hu moments~\cite{jia_autonomous_2011}

Skeleton information is extracted from the Microsoft Kinect SDK, then Bayesian inference is used to sample over all possible robot poses best suited for an interaction~\cite{mead_probabilistic_2012}.

Unknown techniques:
Trajectories are generated based on an ideal interaction area in front of the detected person~\cite{sisbot_synthesizing_2010}.

Unknown face detection method~\cite{cheng_multiple-robot_2013}

Face regions are detected with the Viola-Jones method from OpenCV, then an online random ferns method compares pixel intensities to learn a particular persons face~\cite{ferrer_robot_2013}. This method also utilises human feedback (through a keyboard and touch screen) to improve the classifier when the predictions are uncertain.

Weinrich et al~\cite{weinrich_appearance-based_2013} use a laser for leg detect, then use HOG with a sliding window with a multi-resolution pyramid of the input image to identify, and re-identify, the upper body of a detected person compared with an appearance model (manually constructed model of an upper body).


Yun et al~\cite{yun_robotic_2013} use online multiple instance learning (MIL~\cite{babenko_visual_2009}) to track a person from the back appearance, training a colour histogram score from online images using both positive and negative examples. Chen et al~\cite{chen_stereovision-only_2014} also utilise MIL to perform segmentation with skin colour to detect a person, updating the adaptive appearance model of the person and the local image background. 

Weber et al~\cite{weber_follow_2018} used a CNN (VGG-16~\cite{simonyan_very_2015}) with single shot detection (SSD~\cite{liu_ssd_2016}) for head detection. Detections were then tracked with LSD SLAM~\cite{fleet_lsd-slam_2014} and through the fitting of faces to a template face model (3D morphable face model 3DMM).

Face detection is perform using the Viola-Jones method~\cite{do_human-robot_2014}. 

Hu et al use a model of a person walking to anticipate human movement and more accurately perform person following~\cite{hu_design_2014}.

Munaro et al~\cite{munaro_fast_2014} create a voxel grid filter from an RGB-D image to remove the ground, and cluster groups of voxels based on 3D proximity and shape to detect and track people.


Ali et al~\cite{ali_improved_2015} uses the Viola-Jones method for face detection, and a particle filter for target tracking. Laser for leg obstacle avoidance.

Gupta et al~\cite{gupta_robust_2015} first subtract the background, then perform template matching on the segmented image to detect a person. A motion model and Kalman filter result in smooth tracking.

Bayram et al~\cite{bayram_audio-visual_2016} also use the Viola-Jones for face detection, then perform color-based tracking in YCbCr colour space using Camshift in OpenCV.

Hassan et al~\cite{hassan_computationally_2016} requires a person hold a coloured marker. Colour segmentation is performed and following occurs with the aid of a ultra-sonic range sensor.

Voxelisation, segmentation and 3D clustering is used to detect a person when the sensor is moving~\cite{kahily_real-time_2016}.

HOG features into an SVM to determine if there is a leg. Kalman filter for tracking~\cite{talebpour_-board_2016}

People are detected using HOG features into an SVM, and confirmed using height and distance~\cite{vasconcelos_socially_2016}.

Angonese et al~\cite{angonese_multiple_2017} train a GoogLeNet~\cite{szegedy_going_2015} CNN to detect specific instances of people, such that they can be integrated into a SLAM algorithm for robot navigation. Features from the CNN were used with an SVM. This required a custom dataset of people to be collected. The CNN was pre-trained on ImageNet

Viola-jones for face detection and tracking for blimp~\cite{yao_monocular_2017}.

Laser for slam, skeleton for person tracking (OpenNI)~\cite{yuan_development_2018}

Condes et al~\cite{condes_person_2019} first use a single shot detector (SSD) network~\cite{liu_ssd_2016} to detect a person, then use the Viola-Jones method to determine the region of the persons face. Tracking is performed by determining if a detection in a new frame is near the pixel location in a previous frame. Finally, FaceNet~\cite{schroff_facenet_2015}, a CNN that outputs a vector embedding of a face, is used to determine if the face detected is of a known face, and is used for re-identification when a target person is lost.

Luo et al~\cite{luo_real-time_2019} use a kernalised correlation filter (KCF) to track a target across image frames. An extended kalman filter is used to account for the noise of the predictions.

Skeleton information obtained with Kinect SDK, tracking is performed with optic flow~\cite{wu_improved_2019}

OpenPose for skeleton~\cite{yang_socially-aware_2019}, social force model for navigation adhering to social conventions. Laser for obstacles.

A person is detected and tracked using the contours of the target in the image (target contour band)~\cite{zhang_vision-based_2019}. The robot follows the target using image based visual servo control using a kinematic model of the robot and the bounding corners of the target in the image.

SSD for person, FaceNet to detect specific person, KCF for tracking~\cite{hwang_interactions_2020}.

With gestures:
Laser for leg detection, Viola-Jones for face detection and tracking~\cite{pereira_human-robot_2013}.

Body tracking using skeleton extracted from the Microsoft Kinect SDK~\cite{fujii_gesture_2014}

Prediger et al~\cite{prediger_robot-supported_2014} extract a skeleton tracking with particle filter.

Skeleton extraction, Gesture Builder, and Kalman filter~\cite{long_kinect-based_2018}

OpeNI for joint angles, and motion tracking with human motion prediction~\cite{chen_human-following_2019}.

OpenPose for gestures and skeleton~\cite{miller_self-driving_2019}, goals are given in the robot occupancy map that are a fixed offset from the tracked human.

Kinect SDK for skeleton and following~\cite{anuradha_human_2020}.

Colour segmentation~\cite{wu_toward_2020}.

A vision network is used to create an intelligent work space, where a mobile robot can identify and avoid people~\cite{almonfrey_flexible_2018}. Pedestrian detector models. The pedestrian detectors
(ICCF and ACF) were trained with the INRIA dataset~\cite{dalal_histograms_2005}. Bounding box dimensions are used to determine the 3D location of the people and robot in the scene.

Viola-Jones on custom dataset of people (not just face, body poses)~\cite{luo_human_2010}.

% ==================================

How we are classifying RMHS: 

- Mobile robot and the person is passive in the visual exchange (else it would be gesture or action), (examples: following, approaching, avoiding). Can exist with gesture and action, provided RMHS is separate (e.g. the technique hasn't already been mentioned).

ALL MOBILE ROBOTS:

OTHER

Operator in the loop for surveillance mobile robots~\cite{do_human-robot_2014}

GESTURE CONTROL

Mobile robot goes to location pointed to~\cite{martin_estimation_2010, van_den_bergh_real-time_2011, abidi_human_2013, park_real-time_2011}. In the case of ~\cite{van_den_bergh_real-time_2011} pointing occurs from the hand, and the pointing location is added to the robot map for otherwise autonomous exploration. Abidi uses PR-2 in domestic environment. Park uses social robot in domestic environment.

Approaching with handover: Mobile with manipulator, follows user gestures, face, and voice commands, navigates to person, around person, and to area pointed to (table)~\cite{burger_two-handed_2012}. Mobile manipulator hands over water bottle (R2D2 with small robot inside)~\cite{cheng_multiple-robot_2013}.

Examples of state change include initiating person guiding or following~\cite{pereira_human-robot_2013}, or choosing path direction (left or right) of an otherwise autonomous navigating robot~\cite{lalejini_evaluation_2015, ehlers_human-robot_2016}. Service robot goes into follow-me mode, wait, or stop with waving of arms~\cite{fujii_gesture_2014}

~\cite{fareed_gesture_2015} perform obstacle detection and avoidance while responding to gestures commands.

~\cite{jevtic_comparison_2015} perform person following, and compare to pointing.



% Up to here with movement + gesture ==============
~\cite{prediger_robot-supported_2014}
% =================================================

APPROACHING

~\cite{ferrer_robot_2013}

Robot approaches person with face detection~\cite{budiharto_indoor_2010}, with stereo vision ~\cite{chen_stereovision-only_2014}

Engagement detection~\cite{vaufreydaz_starting_2016}



FOLLOWING 

~\cite{alvarez-santos_feature_2012, mead_probabilistic_2012, ali_human_2013, yun_robotic_2013, munaro_fast_2014, gupta_robust_2015, kahily_real-time_2016, talebpour_-board_2016}

Social considerations~\cite{vasconcelos_socially_2016}

With speech as well~\cite{nguyen_audio-visual_2014, bayram_audio-visual_2016}

Person wears haptic band that signals when the human its leaving the path, multiple following robots that use vision~\cite{scheggi_human-robot_2014}

UAV follows a blue gloved hand~\cite{miyoshi_above_2014}, 


Anticipate human behaviour when following~\cite{hu_design_2014}


Person wearing particlar clothing~\cite{chen_person_2012}, or coloured marker~\cite{hassan_computationally_2016} (low computational cost)

Service robot person following ~\cite{fahn_real-time_2010}

Wheelchair and museum robot following, also has laser~\cite{kobayashi_people_2010}

Wheelchair robot following, also use lasers, vision for re-finding person~\cite{wu_accompanist_2012}

Following and re-identification~\cite{weinrich_appearance-based_2013}


Mobile robot with manipulator approaches human and hands over a bottle~\cite{sisbot_synthesizing_2010}

People following with several sensors in addition to vision (speech, IR, ultrasonic)~\cite{yun_robust_2010}

Human following with stereo vision~\cite{jia_autonomous_2011, ali_improved_2015}

Hand tracking for controlling mobile robot~\cite{paulo_vision-based_2012}



APPLICATION AREAS:
===================================================================================================
ACTION RECOGNITION:
===================================================================================================



===================================================================================================
GESTURE RECOGNITION:
===================================================================================================

Number of control papers:
HAND: 11, 5, 4, 8 = 28
Body gestures: 11 + 20 + 12 = 43
Facial expressions: 3
Total = 74

HAND GESTURES

Control: 11

Control: 5
Hand gestures for controlling robot arm with pre-defined responses~\cite{choudhary_real_2015, deepan_raj_static_2017, song_towards_2017}, lego mindstorm~\cite{song_towards_2017}, or for object handover where the robot arm places an object in the persons hand if it is open~\cite{arenas_deep_2017}, or for object selection and confirmation~\cite{vysocky_interaction_2019}

Control: 4
Coupled with joint control where the hand gesture controls the gripper (open or close)~\cite{fareed_gesture_2015, lima_real-time_2019, martin_real-time_2019, luo_human-robot_2019}. Continuous joint control (following human joint position)~\cite{lima_real-time_2019, martin_real-time_2019}, or with body gestures that controls the arm position~\cite{fareed_gesture_2015}. Lifting gripper~\cite{luo_human-robot_2019}.

Control: 8
Wearable cameras attached to a persons wrist that detect hand gestures to control a wheelchair robot~\cite{yang_novel_2018} and a dual arm robot~\cite{chen_wristcam_2019}.

Mobile robot with gripper, two hand gestures, one to move the robot base, and the other to control the gripper~\cite{fareed_gesture_2015, fareeluo_human-robot_2019}. 

Multimodel fusion~\cite{gao_hand_2020}, astronaut hand mimic, MYO sensor. 

Hand pointing (pointing classified just from hand): ~\cite{luo_tracking_2011, ikai_robot_2016, du_online_2018, vysocky_interaction_2019}. 

Hand gestures (including pointing) can be classified by first getting the human pose, then extracting the region of pixels where the hand would be~\cite{van_den_bergh_real-time_2011}.

% --------------------------------
% Not control:
Hand gestures for playing paper scissors rock~\cite{katsuki_high_speed_2015, yuan_natural_2020}.

Hand gestures for interacting with social robot (humanoid)~\cite{ju_integrative_2017}

Hand gestures can be used to program a robot, such as in the work by Mazhar et al~\cite{mazhar_real-time_2019}, where a pre-determined hand gesture signifies the recording of a task. The robot becomes compliant once the command has been received so the human programmer can manually move the robot end effector to perform a desired action. A second gesture determines the completion of programming, and the robot begins executing the new task. 

An industrial robot arm tracks hand position while learning from online demonstrations. When the robot gets close to the desired position, fine tuning is performed by speech and static hand gesture pointing~\cite{du_online_2018}.

A humanoid robot (Pepper and NAO) detects and tracks a human, then identifies gestures (fingerspelling), then performs a gesture response for communication with deaf-mute people, tested in a public service centre where 9/10 people preferred an embodied robot over a virtual robot on a screen~\cite{kalidolda_towards_2018}.

BODY GESTURES

% Static gesture (pointing, hand gestures), dynamic gesture such as waving (Nao robot on mobile base, waves back, and goes to object pointed to)~\cite{canal_gesture_2015}.

POINTING = 3 hand + 19 from body = 22
WAVING = 7
Body pose control: 11 + 20 + 12

% -------------------------------------
Control: 11
Pointing gestures for controlling mobile robots~\cite{park_real-time_2011, van_den_bergh_real-time_2011, yoshida_evaluation_2011, abidi_human_2013, nishiyama_human_2013, prediger_robot-supported_2014, chen_stereovision-only_2014, jevtic_comparison_2015, tolgyessy_foundations_2017, chen_human-following_2019}. Pointing with two hands~\cite{burger_two-handed_2012}. 

Control: 20
Pointing for robot selection in multi-robot team, UAV:~\cite{lichtenstern_prototyping_2012}, mobile robot ~\cite{milligan_selecting_2011}, multi-robot team (closes robot goes to pointing location)~\cite{nishiyama_human_2013}.

Pointing at an object for mobile robot with manipulator to pick up~\cite{droeschel_towards_2011, moh_gesture_2019, sriram_mobile_2019}, 

robot confirms object by also pointing~\cite{quintero_visual_2015}.

Body gesture control of mobile robot with pre-defined responses~\cite{fujii_gesture_2014,xu_online_2014, cicirelli_kinect-based_2015,fareed_gesture_2015,lalejini_evaluation_2015, ghandour_human_2017,long_kinect-based_2018, pentiuc_drive_2018, zhang_interactive_2018, zhang_automating_2018, chen_human-following_2019,miller_self-driving_2019, kahlouche_human_2019}, (e.g. waving gestures for follow-me, bye-bye)~\cite{fujii_gesture_2014}, turn left/right~\cite{lalejini_evaluation_2015}, and drawing shapes with hands~\cite{xu_online_2014}. Shoulder angle used to control heading angle of a mobile robot with discrete angles (45 degree increments)~\cite{wang_wheeled_2013}. Body gesture control of otherwise autonomous mobile robot (turn, stop)~\cite{ghandour_human_2017}, or when to start or stop following (a nurse in an hospital setting)~\cite{long_kinect-based_2018}, or for an autonomous ottoman that determines if a user would like to put their feet up~\cite{zhang_automating_2018}. Another following robot that changes state with gestures~\cite{chen_human-following_2019}. Tracked robot forward/backwards/left/right from body gestures~\cite{fang_vehicle-mounted_2019}. Following and parking behaviour with body gestures~\cite{miller_self-driving_2019}. Mobile robot approaches human with waving gesture, stops where pointed~\cite{kahlouche_human_2019}

Control: 12
A wheelchair robot velocity is commanded by human shoulder position, and changes configuration (bed mode and sitting mode) with body gesture~\cite{mao_medical_2018}

Mobile robot with manipulator picks up object pointed to~\cite{qian_visually_2013}.

Select mobile robot by looking directly at it in a multi-robot team, with optic-flow to classify waving gesture to determine where the robot should move to~\cite{couture-beil_selecting_2010}. Multiple UAV's detect a persons face direction, robot selection is performed when the person waves to a robot it they are looking at, deselection occurs when they wave with the opposite hand. The selected robots then respond to a command (e.g. land)~\cite{monajjemi_hri_2013}

Direct joint control of humanoid upper body, plus body gestures (rotate the torso, move one foot forward or backward) to control mobile base~\cite{broccia_gestural_2011}. Humanoid (Nao) on mobile base, Nao waves if human waves, mobile base goes to location pointed to~\cite{canal_gesture_2015}.

Body gesture control of humanoid with pre-defined response (e.g. walking)~\cite{shieh_fuzzy_2014,gao_humanoid_2015,han_human_2017}.

Multiple robots, where one robot observes the pointing gesture and communicates with the robot target (UAV's)~\cite{lichtenstern_prototyping_2012}, or to the closest mobile robot to the pointing target~\cite{nishiyama_human_2013}.

Swarm pattern control of multiple robots with gestures. Body pose (arms out, above head), signify different configurations of (little robots make a surprised or happy face)~\cite{alonso-mora_human_2014}.
% -------------------------------------
% Not control:
Programming an industrial robot arm with body gestures~\cite{stipancic_programming_2012}, and hand gestures~\cite{mazhar_real-time_2019}.

Robot provides feedback for human performing pose from exercise program ~\cite{werner_evaluation_2013, gorer_autonomous_2017,  avioz-sarig_robotic_2020} (Nao robot, poppy robot).

Mobile robot approaches human after inferring user intent through body pose and facial expressions~\cite{li_inferring_2019}

HEAD GESTURES
control: 3
Robot head (Eddie) mimic facial expressions~\cite{sosnowski_mirror_2010}, Alice~\cite{meghdari_real-time_2017}, reeti~\cite{masmoudi_expressive_2011}

Interest detection from head gestures (shaking, nodding head), static (head up or down) for social interaction with humanoid upper body~\cite{saleh_nonverbal_2015}.

Robot head performs set of facial expressions for human classification (e.g. if human sad, robot will be surprised, then sad)~\cite{ke_vision_2016}

Social interaction by detection facial expressions (respond depending on expression) HAAR features for detecting face region, then CNN and LSTM. Use fine-tuning from a pre-trained network.~\cite{li_cnn_2019}

Engagement detection from facial expression recognition~\cite{castellano_context-sensitive_2014}.





===================================================================================================
\subsubsection{Object Handover and Collaborative Actions}
===================================================================================================
% Robot counts:
% UR series of robot arm (n=4), others include Kuka (n=5), ABB (n=3), SCARA (n=1), Staubili (n=2), Baxter (n=2), Sawyer (n=1), Frankas Panda arm (n=3), Lab-Volt 5150, ASIMO, Jido, Adept Cobra s800, Kawasaky RS005LA, WAM robot arm = 17 singles/unknowns

Safe workspace ~\cite{nair_3d_2011}

Industrial arm moves Tool Center Point (TCP) to mimic human hand~\cite{christiernin_interacting_2016}, Asimo moves end effectors to mimic human hand position~\cite{arumbakkam_multi-modal_2010}

Approaching with handover: Mobile with manipulator, follows user gestures, face, and voice commands, navigates to person, around person, and to area pointed to (table)~\cite{burger_two-handed_2012}. Mobile manipulator hands over water bottle (R2D2 with small robot inside)~\cite{cheng_multiple-robot_2013}.

===================================================================================================
\subsubsection{Learning from Demonstration}
===================================================================================================

===================================================================================================
\subsubsection{Social Classification and Communication} 
===================================================================================================



===================================================================================================
USER STUDIES: see User Studies spreadsheet
===================================================================================================
Action recognition:
~\cite{lee_learning_2017, efthymiou_multi-_2018, sorostinean_activity_2018, lang_research_2020}

Gesture recognition:
~\cite{martin_estimation_2010, park_real-time_2011, yoshida_evaluation_2011, faudzi_real-time_2012, gori_all_2012, abidi_human_2013,werner_evaluation_2013,castellano_context-sensitive_2014, fujii_gesture_2014, prediger_robot-supported_2014, canal_gesture_2015, gao_humanoid_2015, jevtic_comparison_2015, lalejini_evaluation_2015, saleh_nonverbal_2015, ehlers_human-robot_2016, ghandour_human_2017, gorer_autonomous_2017, han_human_2017, kalidolda_towards_2018, yuan_development_2018, zhang_automating_2018, li_inferring_2019, lima_real-time_2019, avioz-sarig_robotic_2020, yuan_natural_2020}

Robot movement:
~\cite{martin_estimation_2010,park_real-time_2011,yoshida_evaluation_2011,ferrer_robot_2013,abidi_human_2013, scheggi_human-robot_2014,fujii_gesture_2014, prediger_robot-supported_2014,canal_gesture_2015,jevtic_comparison_2015, lalejini_evaluation_2015, ehlers_human-robot_2016, mollaret_multi-modal_2016, ghandour_human_2017, yuan_development_2018, zhang_automating_2018, li_inferring_2019}

Object Handover and Collaborative Actions
~\cite{christiernin_interacting_2016, lee_learning_2017, kogkas_free-view_2019, lima_real-time_2019, valle_personalized_2019, arai_service_2020}

Social:
~\cite{foster_two_2012, gori_all_2012,werner_evaluation_2013, castellano_context-sensitive_2014,taheri_social_2014,  gao_humanoid_2015, li_visual_2015, saleh_nonverbal_2015, mollaret_multi-modal_2016, bilac_gaze_2017, gorer_autonomous_2017, efthymiou_multi-_2018, kalidolda_towards_2018, sorostinean_activity_2018, avioz-sarig_robotic_2020, lang_research_2020, yuan_natural_2020}

==> ExtraFiles/scratchpad_themes.tex <==
meta themes, what are additional trends are we seeing:
- Cost of sensors, processing speed
- Accessibility of sensors and off-the-shelf algorithms (kinect with skeletons)
- Datasets: very little benchmarking of vision techniques against known datasets


==> ExtraFiles/section2B_old.tex <==

The following section provides a detailed review for robotic vision techniques used in each application area. In this section, we present information on the process of robotic vision, including algorithms, data sets, cameras and methods to allow robots to provide information, support or actions via robotic vision. 


% ==============================================================
\subsection{Gesture Recognition}
% ==============================================================

Gesture recognition via robotic vision involves being able to identify hand and body gestures from video streams. Robotic vision for gesture recognition is commonly performed using a two-step process. First, there is an extraction step in which the hand, body or head is identified in an image. Second, a classification step is performed to determine what gesture is being demonstrated by the human. Here we will discuss the two steps in detail and common techniques used within each domain for gesture recognition. 

%\subsubsection{Step 1 - Extraction Step - Process, Techniques, Methods:} 
\subsubsection{Overview:} 

To start the process of gesture recognition, the first step is often to first extract the hand, body or head from the image. This includes finding the location of the human in the image, and seeking to detect a human face in the image or video stream. To detect a human face, the Viola-Jones method~\cite{viola_robust_2004} was commonly used for this step ~\cite{couture-beil_selecting_2010, martin_estimation_2010, droeschel_towards_2011, lam_real-time_2011,  van_den_bergh_real-time_2011,pereira_human-robot_2013, monajjemi_hri_2013}. The Viola-Jones method involves using Haar filters to extract features from an image, and AdaBoost to make predictions based on a weighted sum of features. Finally, a cascade of classifiers makes the algorithm more efficient by discarding false detections early. Face location can also be used as a method to help determine where in the image the algorithm should focus on to increase the chance of detecting the location of the persons hands ~\cite{droeschel_towards_2011, luo_tracking_2011, milligan_selecting_2011}. Colour segmentation was often used to find a hand in an image. This included where the human was required to wear a coloured item (for example a coloured glove~\cite{chen_integrated_2010, yoshida_evaluation_2011, faudzi_real-time_2012}, a piece of coloured clothing~\cite{hassan_computationally_2016}, or with coloured tape around specific fingers~\cite{lavanya_gesture_2018}). Colour segmentation has also been used to segmenting skin tone~\cite{chen_approaches_2010, manigandan_wireless_2010, luo_tracking_2011, park_real-time_2011}. Segmentation is typically performed in HSV~\cite{manigandan_wireless_2010, lambrecht_spatial_2012, raajan_hand_2013, sriram_mobile_2019}, or YCrCb~\cite{luo_tracking_2011, choudhary_real_2015, xu_skeleton_2020} colour spaces, using hand coded threshold values~\cite{chen_approaches_2010, luo_tracking_2011, raajan_hand_2013, choudhary_real_2015}, or by using histogram analysis from a skin sample~\cite{manigandan_wireless_2010, lambrecht_spatial_2012, xu_skeleton_2020}. Segmentation is also performed with the aid of the depth sensors~\cite{droeschel_towards_2011, paulo_vision-based_2012, mazhar_real-time_2019, xu_skeleton_2020}. Droschel et al~\cite{droeschel_towards_2011} apply 3D region growing using the centroid of the head as a seeding point. Paulo et al~\cite{paulo_vision-based_2012} segment hand gestures by setting minimum and maximum distances to the sensor. Mazhar et al~\cite{mazhar_real-time_2019} first extract hand position using skeleton information, then find the bounding region of the hand using depth. Xu et al~\cite{xu_skeleton_2020} perform colour segmentation thresholds tuned for human skin tone, and incorporate depth to remove segmentation errors. Skeleton tracking was commonly used to extract human features from an image, using RGB-D cameras (example papers include~\cite{broccia_gestural_2011, lichtenstern_prototyping_2012, cicirelli_kinect-based_2015,fang_vehicle-mounted_2019, chen_human-following_2019, kahlouche_human_2019}, and RGB cameras (for example with OpenPose~\cite{Cao_2017_CVPR})~\cite{martin_real-time_2019, mazhar_real-time_2019, miller_self-driving_2019}. 

% Skeleton information was then used to extract image regions for hand gesture detection~\cite{lima_real-time_2019}, or to classify body gestures from human joint positions. or by using a secondary detector to first identify the location of the human and sampling coloured pixels from this region (for example by first detecting the head)~\cite{}

%\subsubsection{Step 2 - Classification Step - Process, Techniques, Methods:}

Once the region of interest is extracted, hand and body gestures are classified through a variety of methods depending on the dynamic or static nature of the gestures being performed. For static hand gestures, classification was often performed from segmented images by determining the contours (boundary pixels of a region) and the convex hull (smallest convex polygon to contain the region) as a method of counting the number of fingers being held up~\cite{lambrecht_spatial_2012, raajan_hand_2013, choudhary_real_2015, deepan_raj_static_2017,  sriram_mobile_2019, xu_skeleton_2020}. The distance of each contour point to the centroid of the segmented image was also used for finger counting~\cite{manigandan_wireless_2010, luo_tracking_2011}. From skeleton information, gestures were often classified from the 3D joint positions of the human skeleton using the angular configuration of the joints~\cite{cheng_design_2012, lichtenstern_prototyping_2012, nishiyama_human_2013, wang_vision-guided_2013, fujii_gesture_2014, yang_real-time_2015, fareed_gesture_2015, han_human_2017, miller_self-driving_2019, moh_gesture_2019}, or by using add-on SDK's (such as Visual Gesture Builder~\cite{long_kinect-based_2018}, OpenNI User Generator~\cite{yuan_development_2018}, and the supporting SDK for the Intel Realsense~\cite{vysocky_interaction_2019}). Ghandour et al~\cite{ghandour_human_2017} train a neural network classifier for body pose gestures, using joint positions as input that were first extracted from skeletal information. Li et al~\cite{li_real-time_2019} provide an LSTM network with joint positions to determine the users intention.

% other
% and using classification algorithms such as support vector machines (SVM)~\cite{ehlers_human-robot_2016} and neural networks~\cite{cicirelli_kinect-based_2015, ghandour_human_2017}. 

% Histograms of Oriented Gradients (HOG)~\cite{gori_all_2012}, , SIFT

% Historgram of flow~\cite{gori_all_2012}?. 

% Parallel Tracking and Mapping (PTAM)~\cite{monajjemi_hri_2013}

Dynamic gestures that require a sequence of gestures for classification use multiple image frames. Common algorithms used to track and classify dynamic gestures include Hidden Markov Models (HMM)~\cite{park_real-time_2011, droeschel_towards_2011, burger_two-handed_2012, tao_multilayer_2013, fujii_gesture_2014, xu_online_2014}, optic flow for hand wave detection~\cite{monajjemi_hri_2013}, particle filters for tracking face and hands~\cite{park_real-time_2011, burger_two-handed_2012, prediger_robot-supported_2014, du_online_2018}, and Dynamic Time Warping (DTW)~\cite{qian_visually_2013, canal_gesture_2015, vircikova_teach_2015, pentiuc_drive_2018, chen_wristcam_2019}. Tao et al~\cite{tao_multilayer_2013} use a neural network to segment 3D acceleration and 3D angular
velocity data of hand gestures into a binary gesture indication value, and use a HMM to classify hand waves in various directions. Chen et al~\cite{chen_wristcam_2019} compare SURF features between frames to determine the background velocity from a wrist mounted camera, then perform DTW to classify dynamic hand gestures. Using the joint positions and a fast Fourier transform (FFT) to extract a sequence of feature vectors, Cicirelli et al~\cite{cicirelli_kinect-based_2015} train a separate neural network for each of the ten recognised body gestures. The input to this network is three features (elbow angle, and shoulder angles in two planes) for 60 frames. 

Other classification methods used traditional machine learning techniques, such as k-nearest neighbors (k-NN)~\cite{pereira_human-robot_2013, gao_humanoid_2015, chen_wristcam_2019}, support vector machines (SVM)~\cite{chen_integrated_2010, chen_approaches_2010, gori_all_2012, ehlers_human-robot_2016}, and multi-layered perceptrons (MLP)~\cite{martin_estimation_2010, tao_multilayer_2013}. k-NN was used to determine if a query sample was close to a known set of gestures, where sample features included joint positions,~\cite{gao_humanoid_2015}, Hu moments~\cite{pereira_human-robot_2013}, and velocity vectors found with dynamic time warping (DTW)~\cite{chen_wristcam_2019}. Features classified using an SVM include segmented images~\cite{chen_approaches_2010}, fourier descriptors of image boundaries~\cite{chen_integrated_2010}, and joint position vectors~\cite{ehlers_human-robot_2016} . Other methods use feature extractors such as Haar filters ~\cite{van_den_bergh_real-time_2011} or Gabor filters~\cite{martin_estimation_2010}. Van den bergh~\cite{van_den_bergh_real-time_2011} perform Average Neighborhood Margin Maximization (ANMM) to reduce the dimensionality of of features extracted using Haar filters, and then perform an nearest neighbours comparison to a database of hand gestures. Martin et al train a multi-layer perceptron using features from Gabor filters to recognise pointing gestures~\cite{martin_estimation_2010}. 

Deep neural networks have been adopted for gesture classification with increased popularity in recent years. Convolutional neural networks (CNN's) were used to classify gestures directly from pixels~\cite{arenas_deep_2017, mazhar_real-time_2019, xu_skeleton_2020}, depth images~\cite{kalidolda_towards_2018, lima_real-time_2019}, or from a combination of input channels~\cite{gao_hand_2020}. Neural networks have also been used to perform gesture classification from the skeletal information~\cite{cicirelli_kinect-based_2015, ghandour_human_2017, kahlouche_human_2019, li_real-time_2019}, and other sensory inputs~\cite{martin_estimation_2010, tao_multilayer_2013}. Examples of papers that investigate their own network architecture include~\cite{cicirelli_kinect-based_2015, arenas_deep_2017, ghandour_human_2017, lima_real-time_2019}, and examples where existing network architectures are used include~\cite{mazhar_real-time_2019, waskito_wheeled_2020, gao_hand_2020, xu_skeleton_2020}. Papers that used existing network architectures start with pre-trained models that are then fine tuned on task specific data~\cite{mazhar_real-time_2019}, or train from scratch with a custom dataset~\cite{gao_hand_2020, xu_skeleton_2020, waskito_wheeled_2020}. Mazhar et al~\cite{mazhar_real-time_2019} use a pre-trained Inception V3~\cite{szegedy_rethinking_2016} and fine tune with collected data of hand gestures. Waskito et al~\cite{waskito_wheeled_2020} classify hand gestures from a small amount of collected data (1000 images) by first extracting the binary image of the hand region. Gao et al~\cite{gao_hand_2020} train two Inception V4~\cite{szegedy_incept_2017} networks in parallel, where the input to one network is the full resolution input, and the input to the second network is a low resolution form of the input. This work utilises an Myo arm band, and fuses the RGB, depth, and sEMG data creating a 5 channel image as input. Xu et al~\cite{xu_skeleton_2020} train a ResNet~\cite{he_deep_2016} to learn the minimum convex hull of a hand gesture to determine the number of fingers held up to the robot. Kahlouche et al~\cite{kahlouche_human_2019} fuse multiple classification methods (SVM, decision tree, and a MLP) using a voting process from an ensemble of classifiers. Body pose classifiers with neural networks are used for static~\cite{ghandour_human_2017} and dynamic~\cite{cicirelli_kinect-based_2015, li_cnn_2019} body poses.


\subsubsection{Cameras:}
Gesture recognition can be performed using a variety of different camera systems. Depth aware cameras were used in 59 of the 88 gesture recognition applications identified. Of the 59 papers that used depth aware cameras, 53 of these were the Microsoft Kinect. Single camera set-ups were found in 26 papers. Stereo cameras were used in 5 papers, and omni-directional vision was used in one example. 


\subsubsection{Datasets/Models:} 
Gesture recognition often uses large datasets that involve people in frame performing common and unique gestures for training. Datasets involved videos with xxx and xxx. Common high-quality data sets used in the training session involved xxx, xxx and xxx, which contained xxx(s) video samples that has been pre-cleaning using xxx, and xxx. 

Datasets were most often collected by the researchers using the robotic platform being investigated (key examples include~\cite{martin_estimation_2010, droeschel_towards_2011,park_real-time_2011, pereira_human-robot_2013, tao_multilayer_2013, cicirelli_kinect-based_2015, arenas_deep_2017, ghandour_human_2017, lima_real-time_2019, kahlouche_human_2019, chen_wristcam_2019, xu_skeleton_2020}). Several papers built on previous work for gesture recognition models (the details of datasets used in training were not provided)~\cite{couture-beil_selecting_2010, quintero_visual_2015, ehlers_human-robot_2016, maurtua_natural_2017, martin_real-time_2019, li_real-time_2019}. Papers with datasets made publicly available include~\cite{mazhar_real-time_2019, lima_real-time_2019}. Mazhar et al~\cite{mazhar_real-time_2019} made their dataset of hand gestures `OpenSign' available to others (10 volunteers who recorded 10 static gestures). Lima et al~\cite{lima_real-time_2019} make available their dataset of 160,000 samples from men and women in different poses performing open and closed hand gestures. 

% Do we care about custom dataset sizes? particularly if not released?
% Collected dataset sizes (where reported): 6,000 images~\cite{chen_integrated_2010}, 1,710 images,~\cite{martin_estimation_2010}, 1656 and 348 pointing gestures are used for training and testing.~\cite{park_real-time_2011}, 2082 gesture frames and 61 gestures, 27 of them being static gestures and the other 34 dynamic gestures."~\cite{canal_gesture_2015}, 180 images (for kNN classifier)~\cite{gao_humanoid_2015}, 600 images single background + 1400 images different background~\cite{arenas_deep_2017}, 448 images."~\cite{ghandour_human_2017}, 10,000 training images and 3,500 testing images, all the images are 96*96 gray level images. 5 gestures~\cite{song_towards_2017}. 6000 images (6 gestures).~\cite{waskito_wheeled_2020}. 2500 gesture images.~\cite{xu_skeleton_2020}. 1000 gestures images.~\cite{yang_novel_2018}. 160,000 samples from 20 individuals (15 men and 5 women), hand poses: open and closed hand. ~\cite{lima_real-time_2019}. 30 different people performing 33 manual gestures once. We additionally collected customized data where one person performed the same 33 gestures ten times.~\cite{kalidolda_towards_2018}

% Datasets that use video~\cite{chen_wristcam_2019}. 1350 gestures (135 videos × 10 gestures/video. 15 subjects of 7 females and 8 males. Their ages ranged from 20 to 65 years~\cite{chen_wristcam_2019}. 


\subsubsection{Multiple-Sensors/Sensor Fusion:} Robotic vision for gesture recognition was also paired with other sensor modalities to improve interaction and collaborative processes. Sensors that improve the robot perception of the interaction include speech recognition~\cite{burger_two-handed_2012, fujii_gesture_2014, vysocky_interaction_2019, yuan_development_2018, du_online_2018, maurtua_natural_2017}, surface electromyographic (sEMG) sensor (the Myo gesture control arm band)~\cite{gao_hand_2020}, Leap Motion sensor~\cite{kalidolda_towards_2018}, IMU~\cite{du_online_2018}, and wearable sensors such as a camera attached to a persons wrist to detect hand gestures are used to control a dual arm robot~\cite{chen_wristcam_2019}. Other modalities provide feedback to the human, including speech response~\cite{kahlouche_human_2019,mazhar_real-time_2019, avioz-sarig_robotic_2020}, LED's that change colour in response to commands~\cite{milligan_selecting_2011, alonso-mora_human_2014}, and a display to provide decision support for operators~\cite{lambrecht_spatial_2012, sriram_mobile_2019, lalejini_evaluation_2015}, such as robot state information~\cite{chen_human-following_2019}. 

% ==================================================
\subsection{Action Recognition}
% ==================================================

Action recognition via robotic vision involves being able to identify human motion from video streams. Similar to gesture recognition, robotic vision for action recognition is commonly performed using a two-step process. First, there is an extraction step in which the body pose is identified in an image. Second, a classification step is performed to determine what action is being demonstrated by the human. Here we will discuss the two steps in detail and common techniques used within each domain for action recognition. 

%\subsubsection{Step 1 - Extraction Step - Process, Techniques, Methods:} 

Actions are recognised by first extracting the relevant human information from the image. Like to gesture recognition, skeleton information is often extracted first, then classification is performed using the position of the extracted joints~\cite{werner_evaluation_2013, gorer_autonomous_2017, avioz-sarig_robotic_2020, lang_research_2020}, or by utilising joint position information with other classification methods~\cite{potdar_learning_2016, sorostinean_activity_2018, chalvatzaki_learn_2019, lang_research_2020}. Alternatively, regions of interest can be acquired using modern deep learning techniques such as faster R-CNN~\cite{renNIPS15fasterrcnn} (used by ~\cite{kollmitz_deep_2019}). Colour segmentation is also used in action recognition to identify where a hand is in an image~\cite{wang_collision-free_2017}. 

%\subsubsection{Step 2 - Classification Step - Process, Techniques, Methods:}

Gorer et al~\cite{gorer_autonomous_2017} compare the joint position of  motion identifier joints and those from a human demonstrator, to identify the disparity from an elderly user performing an exercise pose. The robot also performs face tracking (from on board software) and eye blinking (with changes to eye LED's).

Kollmitz et al\cite{kollmitz_deep_2019} use a Kalman filter to track regions of interest (extracted with faster R-CNN~\cite{renNIPS15fasterrcnn}), and a hidden markov model (HMM) to classify the class label, 3D position and velocity of a person using a walking aid. A ResNet-50~\cite{he_deep_2016} was pre-trained on ImageNet data, using RGB images as input.

Chalvatzaki et al~\cite{chalvatzaki_learn_2019} show that a neural network policy with LSTM cells trained using model based reinforcement learning outperforms several alternative methods (inverse reinforcement learning, model predictive control, and kinematic solutions) when predicting human motion when walking behind a robotic rollator. The policy utilises leg information from laser data, and upper body joint positions extracted from an RGB-D image using OpenPose~\cite{Cao_2017_CVPR}.

Potdar et al~\cite{potdar_learning_2016} reduce the dimensionality of the extracted skeletal information from 60 to 7 using principle component analysis (PCA), then train a LSTM neural network classifier. 

Wang et al use a pre-trained CNN (VGG-16~\cite{simonyan_very_2015}) to extract visual features from an image region and predict hand movement (change in x,y position) using an LSTM model~\cite{wang_collision-free_2017}.

Dense trajectories~\cite{wang_action_2011} are should to provide better features (resulting in more accurate action classifications), than CNN's where there is a mismatch between training and testing data (for example, when identifying the actions of children when large action recognition datasets are of adults)~\cite{efthymiou_multi-_2018}. 

Gui et al train a Generative Adverserial Network (GAN) from motion input (sequence of skeletal data)~\cite{gui_teaching_2018}. Skeleton information is first extracted using OpenPose~\cite{Cao_2017_CVPR} from RGB data. Depth information is then introduced to determine the 3D joint locations. A GAN framework with a single GRU cell for each the encoder and decoder is utilised to generate motion predictions.

Sorostinean et al~\cite{sorostinean_activity_2018} pre-train a LRCN network (Long-term Recurrent Convolutional Network) using the NTU RGB-D dataset~\cite{shahroudy_ntu_2016}, and fine tune with collected data that includes thermal information. First, joint positions were extracted using the Kinect API, then the LRCN network was used to extract features from skeleton information and the depth image. Features from face temperature were also tracked between frames. Features from the depth, skeletal, and thermal information were then used by a support vector machine (SVM) model with a radial bases function (RBF) kernel to classify the actions.

Zhang et al~\cite{zhang_automating_2018} predict if a person is sitting or standing, facing the robot, and if the person is exhibiting a welcoming action (such as waving or stretching). The Microsoft SDK is used to extract skeleton information, then sitting is determined if the skeleton height is less than the height of the standing skeleton, body orientation is determined from shoulder positions, and template matching is used to determine a welcoming pose.

From the skeleton information (extracted from Baidu AI), Lang et al~\cite{lang_research_2020} find the average of 7 key locations (top of the head, left/right elbow, wrist and ankle). These average values were collated to determine an identifier score, with each action corresponding to a unique identifier score.

In the work by Lee et al~\cite{lee_real-time_2020} joint pose information was first extracted from OpenPose~\cite{Cao_2017_CVPR} from RGB data. An image is then create mapping joint positions $x,y,z$ into RGB colour space (each pixel represents a joint location, normalised to be between 0 and 255). Each image column becomes the location of each joint position, and has a row for each camera frame. This compressed joint information image is then passed into a convolutional neural network (CNN) and trained to predict actions on the NTU RGB-D dataset.



\subsubsection{Cameras Used for Action Recognition:}

From the 15 identified papers that used action recognition, the most common camera type was the RGB-D sensor ($n=13$), followed by monocular RGB cameras ($n=2$). In the 13 papers that used an RGB-D camera, 12 used the Microsoft Kinect. In addition to RGB-D cameras, Sorostinean et al~\cite{sorostinean_activity_2018} also utilise thermal cameras in an action recognition scenario.

\subsubsection{Datasets}

Action recognition classification often required the usage of a large dataset of actions~\cite{wang_collision-free_2017, gui_teaching_2018, sorostinean_activity_2018, kollmitz_deep_2019, lee_real-time_2020}. Two papers~\cite{sorostinean_activity_2018, lee_real-time_2020} used the NTU RGB-D dataset~\cite{shahroudy_ntu_2016}, containing 60 action classes from 56,880 video samples with RGB videos, depth map sequences, 3D skeletal data, and infrared (IR) videos for each sample. The manipulation action dataset (MAD)~\cite{fermuller_prediction_2018} was used by~\cite{wang_collision-free_2017} and contains five different objects with five distinct actions. Each action is repeated five times (a total number of 625 recordings)~\cite{wang_collision-free_2017}. The H3.6M dataset~\cite{ionescu_dataset_2014} has 3.6 million 3D human poses (5 female, 6 male from 4 view points) and was used by~\cite{gui_teaching_2018} to train a motion prediction GAN. Kollmitz et al~\cite{kollmitz_deep_2019} make available their dataset of various mobility levels (wheelchair, walker, walking stick) with over 17,000 annotated RGB-D images.

% For the MBRL training we have employed 5000 frames of tracking data from four patients, while for testing the controller’s performance we have kept 2000 data from one patient unseen to the training set.~\cite{chalvatzaki_learn_2019}



% Efthymiou et al~\cite{efthymiou_multi-_2018} use a pre-trained model on the Sports1M corpus, which is then fine-tune to classify the actions in our database. In addition, since we have limited data, we split each of our videos in 16-long frame clips with the 15 frames overlapping and use thse to fine-tune the network~\cite{efthymiou_multi-_2018}. Other database mentions from~\cite{efthymiou_multi-_2018}: the ActivityNet database [29] contains 15,410 videos of 200 classes for training, Sports1M [30] includes over 1 million videos of 487 classes, and UCF101 [31] contains 13,320 videos from 101 classes.

% ==================================================
\subsection{Robot Movement in Human Spaces}
% ==================================================
TODO ~\cite{bellarbi_social_2017}

Mobile robots that operate in human spaces are required to track people through multiple frames, responding as the person or robot moves through the world. The robot must first detect the person/s and then track their location. In some cases the robot is able to re-acquire a target person when they are no longer in view.

% 12 faces, 8 body pose, 3 ssd/
Face detection is one of the more common approaches to detecting if an image is exclusively a person, and the most common method (explained in detail in Sec 2B: Gesture Recognition) is the Viola-Jones method~\cite{viola_robust_2004}, example usage includes~\cite{budiharto_indoor_2010, luo_human_2010, kobayashi_people_2010, lam_real-time_2011, wu_accompanist_2012, ferrer_robot_2013, pereira_human-robot_2013, do_human-robot_2014, ali_improved_2015, bayram_audio-visual_2016, yao_monocular_2017, condes_person_2019}. Luo et al~\cite{luo_human_2010} train the Viola-Jones method to detect the humans from the upwards view of a low mobile robot (not only to detect faces). Another popular solution for person detection is to use skeleton extraction (for example from the Microsoft SDK, OpenNI, or OpenPose)~\cite{ghandour_human_2017, long_kinect-based_2018, yuan_development_2018, chen_human-following_2019, miller_self-driving_2019, wu_improved_2019, yang_socially-aware_2019, anuradha_human_2020}. This method is particularly useful if gestures are also used in part of the system. The single shot detector CNN~\cite{liu_ssd_2016} was used in more recent papers to extract people from a scene~\cite{condes_person_2019, hwang_interactions_2020}, and faces directly~\cite{weber_follow_2018}. Condes et al~\cite{condes_person_2019} utilise the SSD network~\cite{liu_ssd_2016} to first detect the human, then the Viola-Jones method to detect the face within this region. Weber et al~\cite{weber_follow_2018} used a CNN (VGG-16~\cite{simonyan_very_2015}) with single shot detection (SSD~\cite{liu_ssd_2016}) trained with the HollywoodHeads dataset~\cite{vu15heads} for face detection. Detections were then tracked with LSD SLAM~\cite{fleet_lsd-slam_2014} and by fitting of faces to a template face model (3D morphable face model 3DMM)~\cite{weber_follow_2018}. FaceNet~\cite{hwang_interactions_2020} was used to detect faces~\cite{condes_person_2019}, and to recognise a specific persons face~\cite{hwang_interactions_2020}. Angonese et al~\cite{angonese_multiple_2017} use a pre-trained GoogLeNet~\cite{szegedy_going_2015} CNN that was fine tuned on a custom dataset of specific instances of people, such that detections could be integrated as landmarks in a SLAM algorithm for robot navigation. 

Other detection methods use appearance models to match regions of the image to a model~\cite{weinrich_appearance-based_2013, yun_robotic_2013, chen_stereovision-only_2014}. Weinrich et al~\cite{weinrich_appearance-based_2013} use a laser for leg detection, then use HOG with a sliding window with a multi-resolution pyramid of the input image to identify, and re-identify, the upper body of a detected person compared with an appearance model (a manually constructed model of an upper body). Yun et al~\cite{yun_robotic_2013} use online multiple instance learning (MIL~\cite{babenko_visual_2009}) to track a person from the back appearance, training a colour histogram score from online images using both positive and negative examples. Chen et al~\cite{chen_stereovision-only_2014} also utilise MIL to perform segmentation with skin colour to detect a person, updating the adaptive appearance model of the person and the local image background. 3D voxelisation was used extract human shapes from depth images~\cite{munaro_fast_2014, kahily_real-time_2016}. Munro et al~\cite{munaro_fast_2014} created a voxel grid filter from an RGB-D image to remove the ground, and clustered groups of voxels based on 3D proximity and geometric shape to a person. Kahily et al~\cite{kahily_real-time_2016} relied on the Microsoft SDK to extract skeleton information when the robot was not moving, but found voxelisation, segmentation, and 3D clustering to be the preferred person detection method when the sensor was moving~\cite{kahily_real-time_2016}. Images that are first converted to a local binary patterns (LBP)~\cite{ojala_lbp_2002} can be more robust to lighting~\cite{yun_robust_2010}. Alvarez-Santos et al~\cite{alvarez-santos_feature_2012} use a laser for leg detection, then use weighted image features that include LBP~\cite{ojala_lbp_2002}, canny edge detection~\cite{canny_computational_1986}, and histogram of gradients (HOG~\cite{dalal_histograms_2005}) features for robust person detection. HOG features were also used in support vector machines (SVM) to detect legs~\cite{talebpour-board_2016}, and coupled with height and distance information for robust people detection~\cite{vasconcelos_socially_2016}. Jia et al~\cite{jia_autonomous_2011} use the disparity image from a stereo camera, and a canny edge detector to extract a human shape. Head segmentation is the performed using geometric relationships, and compared to a samples from a model image using Hu moments~\cite{jia_autonomous_2011}. Gupta et al~\cite{gupta_robust_2015} first subtract the background, then perform template matching on the segmented image to detect a person. Ferrer et al~\cite{ferrer_robot_2013} use online random ferns to compares pixel intensities to learn a particular persons face. This method also utilises human feedback (through a keyboard and touch screen) to improve the classifier when the predictions are uncertain~\cite{ferrer_robot_2013}. Almonfrey et al~\cite{almonfrey_flexible_2018} developed a vision network using four static cameras to create an intelligent work space, where a mobile robot can identify and avoid people.

Once a human feature (for example the face) is detected, it must be followed between image frames. Tracking is often performed using a particle filter~\cite{fahn_real-time_2010, kobayashi_people_2010, ali_improved_2015, prediger_robot-supported_2014}, or through optic flow~\cite{wu_improved_2019}. Fahn et al~\cite{fahn_real-time_2010} begin the interaction with a face is in the center of the screen, and track the colour spectrum of the skin and hair using a particle filter. SURF features~\cite{bay_speeded-up_2008} are another method for tracking image features through frames~\cite{wu_accompanist_2012}, where image samples can be provided a priori (for example by showing the robot a pattern the target person is wearing~\cite{chen_person_2012}) or by first detecting the human (for example through face detection), then identifying their clothing for tracking~\cite{wu_accompanist_2012}. Kernalized correlation filters (KCF)~\cite{henriques_high-speed_2015} were also used for tracking~\cite{luo_real-time_2019, hwang_interactions_2020}. Human motion prediction~\cite{hu_design_2014, gupta_robust_2015, chen_human-following_2019}, and robot kinematic models~\cite{zhang_vision-based_2019} were used to perform better tracking. Hu et al~\cite{hu_design_2014} use a model of a person walking to anticipate human movement and more accurately perform person following. Zhang et al~\cite{zhang_vision-based_2019} develop a person detection and tracking method that uses the contours of the target in the image (target contour band). The robot follows the target using image based visual servo control using a kinematic model of the robot and the bounding corners of the target in the image~\cite{zhang_vision-based_2019}. Kalman filters were a common method for minimising tracking errors from noisy sensors and odometry~\cite{gupta_robust_2015, talebpour-board_2016, luo_real-time_2019, long_kinect-based_2018}.

% Re-identification of a lost target was considered by several papers~\cite{luo_human_2010, wu_accompanist_2012, weinrich_appearance-based_2013, condes_person_2019, zhang_vision-based_2019}.
% Re-identify targets section todo


\subsubsection{Cameras Used for Robot Movement in Human Spaces:}

From the 48 identified papers where a robot was required to move in human spaces, the most common camera type was the RGB-D sensor ($n=25$), followed by monocular RGB cameras ($n=16$). In the 25 papers that used an RGB-D camera, 19 used the Microsoft Kinect. Other camera types used were stereo cameras ($n=4$) and omni-directional cameras ($n=3$).


\subsubsection{Datasets/Models:} 

Munaro et al~\cite{munaro_fast_2014} release the Kinect Tracking Precision (KTP) dataset, collected from the Microsoft Kinect and containing 8,475 frames with a total of 14,766 instances of people.

Weber et al~\cite{weber_follow_2018} train a face detection model on the HollywoodHeads Dataset~\cite{vu15heads}, containing annotated head bounding box regions for 224,740 video frames from Hollywood movies.

Ferrer et al~\cite{ferrer_robot_2013} collect a dataset to verify their face detection method (12 sequences of 6 different persons).

Almonfrey et al~\cite{almonfrey_flexible_2018} train a person detectors using the INRIA dataset~\cite{dalal_histograms_2005}, containing over 1800 annotated human images. 
% Almonfrey et al~\cite{almonfrey_flexible_2018} also release a dataset of 6000 annotated images, unclear if this is true (mentioned only in the introduction?).

% ==================================================
\subsection{Object Handover and Collaborative Actions}
% ==================================================
% ===============

The most common person extraction technique used for handovers and collaborative actions was by extracting human joint information, from an RGB-D camera~\cite{christiernin_interacting_2016, wang_vision-guided_2013, morato_toward_2014, cherubini_unified_2015, koustoumpardis_human_2016, moreno_path_2016, araiza-lllan_dynamic_2018, bothe_effective_2018, hong_interactive_2018, landi_prediction_2019, scimmi_experimental_2019, valle_personalized_2019, liu_dynamic_2020, zhang_human_2020, gao_user_2020, chan_collision-free_2020, ferraguti_safety_2020}, or with an RGB camera using OpenPose~\cite{zardykhan_collision_2019, van_den_broek_ergonomic_2020}. More than one RGB-D sensor was used to improve the accuracy of human position identification~\cite{wang_vision-guided_2013, morato_toward_2014, pasinetti_development_2018,  scimmi_experimental_2019, ferraguti_safety_2020}. Filters were also used improve the quality of the detected joints~\cite{koustoumpardis_human_2016, hong_interactive_2018}. Face detection was used in one paper, using the Viola-Jones method to control the heading of a humanoid robot using the head position of a human operator~\cite{arumbakkam_multi-modal_2010}. Attaching coloured markers to a person was used in two papers for person detection and tracking in a shared workspace, where multiple cameras were used to localise the person in 3D space~\cite{tan_safety_2010, ding_optimizing_2011}. Other methods for detecting a person relied on them being a known distance from an RGB-D sensor and applying a distance threshold~\cite{shariatee_safe_2017, bolano_towards_2018}. From segmented images, morphology operations and edge detection was performed to extract the person from the image~\cite{shariatee_safe_2017}. Adaptive thresholding was used to find the pupil position in an eye centered image to detect gaze direction~\cite{arai_service_2020}. HOG descriptors were used with an SVM for person detection in a shared manufacturing cell~\cite{pasinetti_development_2018}.

Modelling of robot motion~\cite{wang_vision-guided_2013} and human motion~\cite{morato_toward_2014, landi_prediction_2019, gao_user_2020} improved the ability for controllers to operate safely in collaborative tasks. Landi et al~\cite{landi_prediction_2019} use a semi-adaptable neural network to model the hand position of the human that minimises jerk and improve collision detection. Gao et al~\cite{gao_user_2020} use a Gaussian mixture model to predict the motion of a human in an assisted dressing task~\cite{gao_user_2020}. Inverse kinematics were used to plan a trajectory that avoids the human~\cite{moreno_path_2016, zardykhan_collision_2019}. Voxelisation of an RGB-D images was also used to help avoid collisions with a person~\cite{mronga_constraint-based_2020, tarbouriech_bi-objective_2020}. Mronga et al~\cite{mronga_constraint-based_2020} use kinematic continuous collision detection (KCCD) to plan a path that avoids contact. Tarbouriech et al~\cite{tarbouriech_bi-objective_2020} use bi-directional RRT with a 3d occupancy grid to plan for human avoidance, and awareness. Visual servoing was used as method to direct a robot to a grasp location in an collaborative manipulation task~\cite{koustoumpardis_human_2016}, or towards the human hand in a handover task ~\cite{bdiwi_handing-over_2013, rosenberger_object-independent_2020}.

Particle filters were used for person tracking between image frames~\cite{arumbakkam_multi-modal_2010, nair_3d_2011, morato_toward_2014}. Nair et al~\cite{nair_3d_2011} track multiple people in an shared workspace by first segmenting the background from a static background model, then matching a fixed size 3D bounding box to segmented region for detection. To reduce computational load with multiple person detections, a global particle set is divided between the number of detections~\cite{nair_3d_2011}. Kalman filters were used~\cite{morato_toward_2014}

Kogkas et al~\cite{kogkas_free-view_2019} use a motion capture system to detect head pose, and eye-tracking glasses for gaze estimation. In a surgical task, a surgeon selects an instrument by looking at the item on a screen for a fixed period~\cite{kogkas_free-view_2019}. Dometrios et al~\cite{dometios_real-time_2017} use a depth camera to extract the surface shape of a human back for a person washing application with a soft robot.

Recent methods use convolutional neural networks (CNN's) for human detection in collaborative tasks. Bingol et al~\cite{bingol_practical_2020} utilises two CNN's: one that takes an image as input to determine the proximity of the person to the robot work area, and one that takes a torque feature matrix to determine if there has been contact made with the robot. Rosenberger et al~\cite{rosenberger_object-independent_2020} use a YOLOv3~\cite{} network for object detection, a fine tuned ResNet50~\cite{} network to segment a human hand from grasping locations on an object, and GG-CNN~\cite{} to to detect grasp locations of the segmented object.

% ==================================================

\subsubsection{Cameras Used for Object Handover and Collaborative Actions:}

From the 38 identified papers where a robot collaborated with a human in an an object handover or action, the most common camera type was the RGB-D sensor ($n=30$), followed by monocular RGB cameras ($n=10$). In the 30 papers that used an RGB-D camera, 22 used the Microsoft Kinect. Four papers ($n=3$) used stereo cameras.


\subsubsection{Datasets/Models:} 

The Ego hand dataset~\cite{} (4800 images of hands) was used to train a hand detector~\cite{rosenberger_object-independent_2020}.



% ==================================================
\subsection{Learning from Demonstration}
% ==================================================

Learning from demonstration tasks often used segmented human joint positions from an RGB-D camera~\cite{stipancic_programming_2012, petric_online_2014, potdar_learning_2016, li_learning_2018, du_online_2018}, or from an RGB camera using OpenPose~\cite{mazhar_real-time_2019}. The Viola-Jones face detection method was used by Yoo et al~\cite{yoo_gaze_2017} for face tracking, and segmentation by pixel values was used by Saegusa et al~\cite{saegusa_cognitive_2011} to determine hand position. Gestures were used to determine the commencement and completion of demonstrations~\cite{stipancic_programming_2012, petric_online_2014, du_online_2018, mazhar_real-time_2019}(methods described in the previous sections). 

Petric et al~\cite{petric_online_2014} control a humanoid end-effector using periodic dynamic movement primitives (DMP~\cite{ijspeert_dynamical_2013}). A person points to the part of the robot movement that needs to adapt, with the gesture defining the direction and magnitude of the new motion, and the robot adjusts its movements in response~\cite{petric_online_2014}. Potdar et al~\cite{potdar_learning_2016} use data collected from an interaction between two people to train an LSTM neural network to learn the complementary robot response to the actions of the person. Li et al~\cite{li_learning_2018} use Gaussian mixture models (GMM) and Gaussian mixture regression (GMR) to model the joint trajectories of a person performing a peg in the hole task. Inverse kinematics is used to translate the trajectories into the robot joint space for an imNEU humanoid robot~\cite{li_learning_2018}. Yoo et al~\cite{yoo_gaze_2017} follows a sequence of actions using gaze for a plant watering task. The robot first detects and tracks the human face and hands, and then uses depth thresholding and a CNN for object detection to determine the next object in the sequence~\cite{yoo_gaze_2017}.

% TODO: more on ~\cite{saegusa_cognitive_2011}.

% ==================================================

\subsubsection{Cameras Used for Learning from Demonstration:}

From the 7 papers identified that required the robot to learn from demonstrations, the most common camera type was the RGB-D sensor ($n=6$), of which 5 where the Microsoft Kinect. One paper ($n=1$) used a monocular RGB camera.

\subsubsection{Datasets/Models:} 


% ==================================================
\subsection{Social Classification and Communication} 
% ==================================================

% TODO fix up ones that have been moved
Joint positions extracted from RGB-D sensor~\cite{igorevich_behavioral_2011, torres_implementation_2012, csapo_multimodal_2012, indrajit_development_2013, yang_study_2013, taheri_social_2014, tseng_multi-human_2014, mollaret_multi-modal_2016, meghdari_real-time_2017, augello_towards_2020, lu_research_2020}

Viola-Jones method for face detection~\cite{csapo_multimodal_2012, saleh_nonverbal_2015}. Saleh et al~\cite{saleh_nonverbal_2015} classify head movements, such as nodding and shaking, using the direction and magnitude pattern (DMP) of depth pixels as features classified with an SVM~\cite{saleh_nonverbal_2015}.

% ==================================================

 iCub gaze controller~\cite{boucher_i_2012}


colour segmentation + blob detection and tracking ~\cite{foster_two_2012}

two cameras and colour segmentation for little uav~\cite{miyoshi_above_2014}.

moving average and butterworth filter for joints from kinect~\cite{taheri_social_2014}.

approaches people after detecting TODO~\cite{tseng_multi-human_2014}

Face Detector [27], Identity Recognition (identity, age, and gender) [28], [29], Face Tracking [30], Sound Recognition [25], Sound Localization and AV Fusion (described in this paper).~\cite{cech_active-speaker_2015}.


Opencv haar features viola-jones and cascades, trained for eye, nose, mouth. Gabor filters, PCA, and SVM~\cite{ke_vision_2016}

Random forests for real time 3D face analysis for line of sight OpenNi for body pose. Detects desire to interact with head/shoulder pose, speech. Voice Activity Detection (VAD). particle swarm optimization inspired tracker, tracking and voice are fused for HMM.~\cite{mollaret_multi-modal_2016}

Minimum Redundancy Maximum Relevance (MRMR)~\cite{vaufreydaz_starting_2016}. 29 interactions with the robot,made by 15 different participants, 5 classes for interact, leave interact etc.. 158000 frames

ROS face recognition package - Viola-jones but using depth to remove false positives based on realistic size of face.~\cite{zhang_optimal_2016}

Train filled pause detector (speech), when detected use peppers gaze detector for 1.5s, make a decision whos turn to speak~\cite{bilac_gaze_2017}

MS SDK + Neural network~\cite{meghdari_real-time_2017}

Velocity (MV) Algorithm and RVM, robust regress-based refining. I think they use an sdk~\cite{zhu_robust_2017}

OpenCV, no details of method used for face detection~\cite{gui_teaching_2018}.

This is in action rec as well~\cite{sorostinean_activity_2018}. pepper robot detects activity and responds with questions and change in state.CNN + LSTM using skeleton data (SDK)

ResNet-10 SSD + OpenFace, pre-trained networks~\cite{cazzato_real-time_2019}.

"Fuzzy combination of depth and sonar. penCV’s
OpenCV’s LPBH (Local Binary Patterns Histogram) face recognizer method"~\cite{chien_navigating_2019}

custom gaze detection  - detection face, detect landmarks on face, eye regions, head pose, pupil centre~\cite{jarosz_detecting_2019}

SSD for face detection, NN- facial recognition model. random forest regression, ~\cite{li_inferring_2019}

HAAr features for detecting face region, CNN and LSTM (custom network, search through parameters)~\cite{li_cnn_2019}

OpenNI~\cite{augello_towards_2020}

From extracted features, classification of gestures was performed with traditional machine learning methods such support vector machines (SVM)~\cite{saleh_nonverbal_2015, ke_vision_2016}. SVM's facial expressions~\cite{sosnowski_mirror_2010, castellano_context-sensitive_2014, ke_vision_2016}.  Other methods use feature extractors such as Gabor filters~\cite{ke_vision_2016}. 
Neural network layers that utilise time-series (such as LSTM) are also used to classify dynamic gestures~\cite{li_cnn_2019}.


Recent works use convolutional neural networks to detect the face region ~\cite{li_inferring_2019, li_cnn_2019}. The face location can be used to then classify facial expressions~\cite{li_cnn_2019},

~\cite{lee_visual_2020}semantic slam

OpenNI~\cite{lu_research_2020},

MS SDK for head pose detection~\cite{phong_vietnamese_2020}

OpenCV 2 cascade face detector, which is based on the Viola and Jones and openCV for locating facial features. Emotion classification ~\cite{masmoudi_expressive_2011}

Deep neural networks have been adopted for gesture classification in recent years. The most common usage was convolutional neural networks (CNN's), classifying gestures directly from pixels. Alternatives perform classification from the extracted skeletal information~\cite{}. architectures and use pre-trained models that are then fine tuned on task specific data~\cite{mazhar_real-time_2019, waskito_wheeled_2020}, or trained with a custom dataset~\cite{gao_hand_2020}. Examples of papers that investigate their own network architecture include~\cite{li_cnn_2019}. Li et al~\cite{li_inferring_2019} TODO: SSD for face detection + other things. Li et al~\cite{li_cnn_2019} use a CNN with LSTM to detect facial expression changes.

\subsubsection{Cameras Used for Social Classification and Communication:}

From the 41 papers identified that required the robot to communicate with a human in an social interaction, the most common camera type was the RGB-D sensor ($n=24$), followed by monocular RGB cameras ($n=15$). In the 24 papers that used an RGB-D camera, 23 used the Microsoft Kinect. Two papers ($n=2$) used a stereo camera.

\subsubsection{Datasets/Models:} 

Papers that used datasets from external sources were most commonly used for facial expression recognition~\cite{sosnowski_mirror_2010, castellano_context-sensitive_2014, ke_vision_2016, li_inferring_2019, li_cnn_2019}. The Cohn-Kanade dataset~\cite{kanade_comprehensive_2000} and its extended form (CK+)~\cite{lucey_extended_2010} was used to train facial expression models~\cite{sosnowski_mirror_2010, ke_vision_2016, li_cnn_2019}. Other datasets include FERET, AffectNet, MMI Face Database, and the Inter-ACT corpus. Several papers built on previous work for gesture recognition models (the details of datasets used in training were not provided)~\cite{saleh_nonverbal_2015}. 

the AffectNet Database contains approx- imately 450,000 + Cohn-Kanade (CK+) dataset includes 123 subjects and 593 image sequences. ~\cite{li_cnn_2019}

Datasets that use video~\cite{meghdari_real-time_2017}
"10 persons, 6 males and 4 females Kinect data output was captured at least for 3 seconds with 30 frame per second rate for each facial expression with different head orientation. Though, each person has a dataset that each frame of data is an array with 17 members."~\cite{meghdari_real-time_2017}

Trained on: Aberdeen Facial Database, GUFD Facial Database, Utrecht ECVP Facial Database + images of laboratory personel using openCV’s LPBH~\cite{chien_navigating_2019}.

WIDER FACE dataset + Kaggle facial expres- sion recognition challenge dataset~\cite{li_inferring_2019}


==> tables/table1_1.tex <==
% \newcommand{\w}{4}
% \begin{tabular}{p{0.35\linewidth} | p{0.6\linewidth} | p{0.6\linewidth}}\toprule
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
% \begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]
\renewcommand{\arraystretch}{1.5}
\begin{table}[!htp]\centering
\caption{Table 1 caption}\label{tab:tablet1}
\scriptsize
% \begin{tabular}{lrrrrrrrr}\toprule
\begin{tabular}{p{0.15\columnwidth} | p{0.05\columnwidth} | p{0.1\columnwidth} | p{0.1\columnwidth} |p{0.1\columnwidth} | p{0.1\columnwidth} | p{0.1\columnwidth} | p{0.1\columnwidth}}\toprule
\textbf{Author} &\textbf{Year} &\textbf{Application Area} &\textbf{Domain Area} &\textbf{Type of Robot} &\textbf{Number of Robots} &\textbf{Role of Human} &\textbf{Number of Humans} \\\midrule
Molina et al~\cite{molina_collaborative_2018} &2018 &Grasping Assistance &Domestic &Jaco arm &Single &Operator &Single \\
Almonfrey et al~\cite{almonfrey_flexible_2018} &2018 &Infrastructure inspection &Industry &Parrot AR. Drone 2.0 &Single &Operator &Multiple \\
Cheng et al~\cite{cheng_multiple-robot_2013} &2013 & & & & & & \\
Farulla et al~\cite{farulla_novel_2015} &2015 & & & & & & \\
Yang et al~\cite{yang_novel_2018} &2018 & & & & & & \\
Luo et al~\cite{Luo} &2019 & & & & & & \\
Foukarakis et al~\cite{Foukarakis} &2016 & & & & & & \\
Bellarbi et al~\cite{Bellarbi} &2016 & & & & & & \\
Zillich et al~\cite{Zillich} &2012 & & & & & & \\
Wu et al~\cite{Wu} &2012 & & & & & & \\
Görer et al~\cite{Görer} &2017 & & & & & & \\
Zhang et al~\cite{Zhang} &2013 & & & & & & \\
Zhang et al~\cite{Zhang} &2018 & & & & & & \\
Castellano et al~\cite{Castellano} &2014 & & & & & & \\
Kollmitz et al~\cite{Kollmitz} &2019 & & & & & & \\
Vasquez et al~\cite{Vasquez} &2017 & & & & & & \\
Liu et al~\cite{Liu} &2019 & & & & & & \\
Giuliani et al~\cite{Giuliani} &2010 & & & & & & \\
Yuan et al~\cite{Yuan} &2017 & & & & & & \\
Stückler et al~\cite{Stückler} &2011 & & & & & & \\
Masmoudi et al~\cite{Masmoudi} &2011 & & & & & & \\
Munaro et al~\cite{Munaro} &2014 & & & & & & \\
Bousquet-Jette et al~\cite{Bousquet-Jette} &2017 & & & & & & \\
Kogkas et al~\cite{Kogkas} &2019 & & & & & & \\
Aranda et al~\cite{Aranda} &2010 & & & & & & \\
Fareed et al~\cite{Fareed} &2015 & & & & & & \\
Schrader et al~\cite{Schrader} &2018 & & & & & & \\
Bdiwi et al~\cite{Bdiwi} &2013 & & & & & & \\
Monajjemi et al~\cite{Monajjemi} &2013 & & & & & & \\
Kahlouche et al~\cite{Kahlouche} &2021 & & & & & & \\
Ali et al~\cite{Ali} &2013 & & & & & & \\
Luo et al~\cite{Luo} &2011 & & & & & & \\
Ali et al~\cite{Ali} &2013 & & & & & & \\
Scheggi et al~\cite{Scheggi} &2014 & & & & & & \\
Zhao et al~\cite{Zhao} &2014 & & & & & & \\
Zhang et al~\cite{Zhang} &2018 & & & & & & \\
Li et al~\cite{Li} &2019 & & & & & & \\
Monajjemi et al~\cite{Monajjemi} &2014 & & & & & & \\
Sriram et al~\cite{Sriram} &2019 & & & & & & \\
Tseng et al~\cite{Tseng} &2014 & & & & & & \\
Burke et al~\cite{Burke} &2013 & & & & & & \\
Chien et al~\cite{Chien} &2019 & & & & & & \\
Por et al~\cite{Por} &2010 & & & & & & \\
Chen et al~\cite{Chen} &2012 & & & & & & \\
Fahn et al~\cite{Fahn} &2010 & & & & & & \\
Gong et al~\cite{Gong} &2018 & & & & & & \\
Sun et al~\cite{Sun} &2019 & & & & & & \\
Ferrer et al~\cite{Ferrer} &2013 & & & & & & \\
Tan et al~\cite{Tan} &2010 & & & & & & \\
Wang et al~\cite{Wang} &2020 & & & & & & \\
Arai et al~\cite{Arai} &2020 & & & & & & \\
Lima et al~\cite{Lima} &2019 & & & & & & \\
Lambrecht et al~\cite{Lambrecht} &2012 & & & & & & \\
Jean-Pierre et al~\cite{Jean-Pierre} &2012 & & & & & & \\
Hsieh et al~\cite{Hsieh} &2015 & & & & & & \\
Limin et al~\cite{Limin} &2017 & & & & & & \\
Erol et al~\cite{Erol} &2020 & & & & & & \\
Wu et al~\cite{Wu} &2020 & & & & & & \\
Droeschel et al~\cite{Droeschel} &2011 & & & & & & \\
Haddadin et al~\cite{Haddadin} &2014 & & & & & & \\
Burger et al~\cite{Burger} &2012 & & & & & & \\
Gao et al~\cite{Gao} &2020 & & & & & & \\
Nguyen et al~\cite{Nguyen} &2015 & & & & & & \\
Phong et al~\cite{Phong} &2020 & & & & & & \\
Lee et al~\cite{Lee} &2020 & & & & & & \\
Wang et al~\cite{Wang} &2013 & & & & & & \\
\bottomrule
\end{tabular}
\end{table}

==> tables/table1_2.tex <==
% \newcommand{\w}{4}
% \begin{tabular}{p{0.35\linewidth} | p{0.6\linewidth} | p{0.6\linewidth}}\toprule
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
% \begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]
\renewcommand{\arraystretch}{1.5}
\begin{table}[!htp]\centering
\caption{Table 1 caption}\label{tab:tablet1}
\scriptsize
% \begin{tabular}{lrrrrrrrr}\toprule
\begin{tabular}{p{0.15\columnwidth} | p{0.05\columnwidth} | p{0.1\columnwidth} | p{0.1\columnwidth} |p{0.1\columnwidth} | p{0.1\columnwidth} | p{0.1\columnwidth} | p{0.1\columnwidth} | p{0.1\columnwidth} }\toprule

\textbf{Author} &\textbf{Year} &\textbf{Application Area} &\textbf{Domain Area} &\textbf{Type of Robot} &\textbf{Number of Robots} &\textbf{Role of Human} &\textbf{Number of Humans} \\\midrule

% Author,Date,Robot Type,Domain,Application Area 1,Application Area 2,Application Area 3,Tax 1.4 -  Ratio of People to Robots,Tax 1.8 - Type of Human-Robot Physical Proximity\\

"Aranda, J.; Vinagre, M.; Martín, E.X.; Casamitjana, M.; Casals, A.~\cite{aranda_friendly_2010}"&2010&Fixed Manipulator&Domestic&Object Handover and Collaborative Actions&&&1&Touching\\
"Arumbakkam, A.K.; Yoshikawa, T.; Dariush, B.; Fujimura, K.~\cite{Arum}"&2010&Mobile Manipulator&Domestic&Robot Movement in Human Spaces&Object Handover and Collaborative Actions&&2&Interacting\\
"Budiharto, W.; Jazidie, A.; Purwanto, D.~\cite{Budi}"&2010&Mobile&Domestic&Robot Movement in Human Spaces&&&1&Approaching\\
"Chen, K.-Y.; Chien, C.-C.; Chang, W.-L.; Teng, J.-T.~\cite{Chen}"&2010&Mobile&Domestic&Robot Movement in Human Spaces&Gesture Recognition&&1&Interacting\\
"Chen, T.-D.~\cite{Chen}"&2010&Mobile&Urban&Robot Movement in Human Spaces&Gesture Recognition&&1&Interacting\\
"Couture-Beil, A.; Vaughan, R. T.; Mori, G.~\cite{Cout}"&2010&Mobile&Urban&Robot Movement in Human Spaces&&&1&Interacting\\
"Fahn, C.-S.; Lin, Y.-T.~\cite{Fahn}"&2010&Mobile&Urban&Robot Movement in Human Spaces&&&1&Interacting\\
"Kobayashi, Y.; Kuno, Y.~\cite{Koba}"&2010&Mobile&Urban&Robot Movement in Human Spaces&&&many to 1&Interacting\\
"Liu, H.; Huo, Z.; Yang, G.~\cite{Liu,}"&2010&Mobile&Urban&Robot Movement in Human Spaces&&&1&Following\\
"Manigandan, M.; Jackin, I.M.~\cite{Mani}"&2010&Mobile&Urban&Gesture Recognition&&&1&Interacting\\
"Martin, C.; Steege, F.-F.; Gross, H.-M.~\cite{Mart}"&2010&Mobile&Domestic&Robot Movement in Human Spaces&Gesture Recognition&&1&Interacting\\
"Sisbot, E.A.; Marin-Urias, L.F.; Broquère, X.; Sidobre, D.; Alami, R.~\cite{Sisb}"&2010&Mobile Manipulator&Domestic&Robot Movement in Human Spaces&Object Handover and Collaborative Actions&&1&Touching\\
"Sosnowski, S.; Mayer, C.; Kühnlenz, K.; Radig, B.~\cite{Sosn}"&2010&&&&&&&\\
"Yun, S.; Kim, C.G.; Kim, M.; Choi, M.-T.~\cite{Yun,}"&2010&Mobile&Domestic&Robot Movement in Human Spaces&&&1&Following\\
"Broccia, G.; Livesu, M.; Scateni, R.~\cite{Broc}"&2011&Mobile Manipulator&Urban&Robot Movement in Human Spaces&Gesture Recognition&&1&Interacting\\
"Ding, H.; Wijaya, K.; Reißig, G.; Stursberg, O.~\cite{Ding}"&2011&Fixed Manipulator&Industrial&Object Handover and Collaborative Actions&&&1&Avoiding\\
"Igorevich, R.R.; Ismoilovich, E.P.; Min, D.~\cite{Igor}"&2011&Social&Domestic&Gesture Recognition&&&1&Interacting\\
"Jia, S.; Zhao, L.; Li, X.; Cui, W.; Sheng, J.~\cite{Jia,}"&2011&Mobile&Urban&Robot Movement in Human Spaces&&&1&Following\\
"Lam, M.C.; Prabuwono, A.S.; Arshad, H.; Chan, C.S.~\cite{Lam,}"&2011&Mobile&Domestic&Robot Movement in Human Spaces&&&1&Interacting\\
"Luo, R.C.; Chang, S.-R.; Yang, Y.-P.~\cite{Luo,}"&2011&Social&Domestic&Social Classification and Communication&Gesture Recognition&&2&Interacting\\
"Milligan, B.; Mori, G.; Vaughan, R.~\cite{Mill}"&2011&Mobile&Urban&Robot Movement in Human Spaces&Gesture Recognition&&1/many&Interacting\\
"Nair, S.; Dean-Leon, E.; Knoll, A.~\cite{Nair}"&2011&Fixed Manipulator&Industrial&Object Handover and Collaborative Actions&&&many /1 &Avoiding\\
"Park, C.-B.; Lee, S.-W.~\cite{Park}"&2011&Mobile&Domestic&Robot Movement in Human Spaces&Gesture Recognition&&1&Interacting\\
"Saegusa, R.; Natale, L.; Metta, G.; Sandini, G.~\cite{Saeg}"&2011&Fixed Manipulator&Domestic&Object Handover and Collaborative Actions&Learning from Demonstration&Action Recognition&1&Interacting\\
"Van Den Bergh, M.; Carton, D.; De Nijs, R.; Mitsou, N.; Landsiedel, C.; Kuehnlenz, K.; Wollherr, D.; Van Gool, L.; Buss, M.~\cite{Van }"&2011&Mobile&Domestic&Robot Movement in Human Spaces&Gesture Recognition&&1&Interacting\\
"Yoshida, K.; Hibino, F.; Takahashi, Y.; Maeda, Y.~\cite{Yosh}"&2011&Mobile&Urban&Robot Movement in Human Spaces&Gesture Recognition&&1&Interacting\\
"Alvarez-Santos, V.; Pardo, X.M.; Iglesias, R.; Canedo-Rodriguez, A.; Regueiro, C.V.~\cite{Alva}"&2012&Mobile&Urban&Robot Movement in Human Spaces&&&1&Following\\
"Boucher, J.-D.; Pattacini, U.; Lelong, A.; Bailly, G.; Elisei, F.; Fagel, S.; Dominey, P.F.; Ventre-Dominey, J.~\cite{Bouc}"&2012&Social&Domestic&Social Classification and Communication&&&1&Interacting\\
"Burger, B.; Ferrané, I.; Lerasle, F.; Infantes, G.~\cite{Burg}"&2012&Mobile Manipulator&Domestic&Robot Movement in Human Spaces&Object Handover and Collaborative Actions&Gesture Recognition&1&Interacting\\
"Chen, W.; Guo, S.~\cite{Chen}"&2012&Mobile&Urban&Robot Movement in Human Spaces&&&1&Following\\
"Cheng, L.; Sun, Q.; Su, H.; Cong, Y.; Zhao, S.~\cite{Chen}"&2012&Social&Domestic&Social Classification and Communication&Gesture Recognition&&1&Interacting\\
"Csapó, A.; Gilmartin, E.; Grizou, J.; Han, J.; Meena, R.; Anastasiou, D.; Jokinen, K.; Wilcock, G.~\cite{Csap}"&2012&Social&Urban&Social Classification and Communication&Gesture Recognition&&1&Interacting\\
"Faudzi, A.A.M.; Ali, M.H.K.; Azman, M.A.; Ismail, Z.H.~\cite{Faud}"&2012&Mobile&Domestic&Robot Movement in Human Spaces&Gesture Recognition&&1&Interacting\\
"Foster, M.E.; Gaschler, A.; Giuliani, M.; Isard, A.; Pateraki, M.; Petrick, R.P.A.~\cite{Fost}"&2012&Social&Urban&Social Classification and Communication&&&2&Interacting\\
"Gori, I.; Fanello, S.R.; Metta, G.; Odone, F.~\cite{Gori}"&2012&Social&Domestic&Social Classification and Communication&Gesture Recognition&&1&Interacting\\
"Lambrecht, J.; Kruger, J.~\cite{Lamb}"&2012&Fixed Manipulator&Industrial&Object Handover and Collaborative Actions&Gesture Recognition&&1&Interacting\\
"Lichtenstern, M.; Frassl, M.; Perun, B.; Angermann, M.~\cite{Lich}"&2012&Drone&Field&Gesture Recognition&&&1&Interacting\\
"Lin, H.; Mei, W.; Zhang, Y.~\cite{Lin,}"&2012&&&&&&&\\
"Mead, R.; Mataric, M.J.~\cite{Mead}"&2012&Mobile&Urban&Robot Movement in Human Spaces&&&1&Interacting\\
"Paulo, T.; Fernando, R.; Gil, L.~\cite{Paul}"&2012&Mobile&Urban&Robot Movement in Human Spaces&&&1&Interacting\\
"Stipancic, T.; Jerbic, B.; Bucevic, A.; Curkovic, P.~\cite{Stip}"&2012&Fixed Manipulator&Industrial&Object Handover and Collaborative Actions&Learning from Demonstration&Gesture Recognition&1&Interacting\\
"Torres, N.A.; Clark, N.; Ranatunga, I.; Popa, D.~\cite{Torr}"&2012&Social&Urban&Social Classification and Communication&Gesture Recognition&&1&Interacting\\
"Wu, B.-F.; Jen, C.-L.; Tsou, T.-Y.; Li, W.-F.; Tseng, P.-Y.~\cite{Wu, }"&2012&Mobile&Urban&Robot Movement in Human Spaces&&&1&Following\\
"Abidi, S.; Williams, M.; Johnston, B.~\cite{Abid}"&2013&Mobile&Urban&Robot Movement in Human Spaces&Gesture Recognition&&1&Interacting\\
"Ali, B.; Iqbal, K.F.; Ayaz, Y.; Muhammad, N.~\cite{Ali,}"&2013&Mobile&Urban&Robot Movement in Human Spaces&&&1&Following\\
"Cheng, C.-Y.; Zhuo, Y.-Y.; Kuo, G.-H.~\cite{Chen}"&2013&Mobile Manipulator&Domestic&Robot Movement in Human Spaces&Object Handover and Collaborative Actions&Gesture Recognition&1&Interacting\\
"Ferrer, G.; Garrell, A.; Villamizar, M.; Huerta, I.; Sanfeliu, A.~\cite{Ferr}"&2013&Mobile&Urban&Robot Movement in Human Spaces&&&1&Approaching\\
"Indrajit, W.; Muis, A.~\cite{Indr}"&2013&Social&Domestic&Gesture Recognition&&&1&Interacting\\
"Nishiyama, T.; Takimoto, M.; Kambayashi, Y.~\cite{Nish}"&2013&&&&&&&\\
"Pereira, F.G.; Vassallo, R.F.; Salles, E.O.T.~\cite{Pere}"&2013&Mobile&Urban&Robot Movement in Human Spaces&Gesture Recognition&&1&Following\\
"Qian, K.; Hu, C.~\cite{Qian}"&2013&&&&&&&\\
"Raajan, N.R.; Raghuraman, S.; Vignesh, T.~\cite{Raaj}"&2013&Mobile&Domestic&Robot Movement in Human Spaces&Gesture Recognition&&1&Interacting\\
"Tao, C.; Liu, G.~\cite{Tao,}"&2013&Mobile&Urban&Robot Movement in Human Spaces&Gesture Recognition&&1&Interacting\\
"Wang, L.; Schmidt, B.; Nee, A.Y.C.~\cite{Wang}"&2013&Fixed Manipulator&Industrial&Object Handover and Collaborative Actions&&&1&Avoiding\\
"Wang, Y.; Song, G.; Qiao, G.; Zhang, Y.; Zhang, J.; Wang, W.~\cite{Wang}"&2013&Mobile&Domestic&Robot Movement in Human Spaces&Gesture Recognition&&1&Following\\
"Weinrich, C.; Volkhardt, M.; Gross, H.-M.~\cite{Wein}"&2013&Mobile&Urban&Robot Movement in Human Spaces&&&1&Following\\
"Werner, F.; Krainer, D.; Oberzaucher, J.; Werner, K.~\cite{Wern}"&2013&Social&Urban&Social Classification and Communication&&&1&Interacting\\
"Yang, N.; Duan, F.; Wei, Y.; Liu, C.; Tan, J.T.C.; Xu, B.; Zhang, J.~\cite{Yang}"&2013&Social&Domestic&Gesture Recognition&&&1&Interacting\\
"Yun, W.-H.; Cho, Y.-J.; Kim, D.; Lee, J.; Yoon, H.; Kim, J.~\cite{Yun,}"&2013&Mobile&Urban&Robot Movement in Human Spaces&&&1&Following\\
"Alonso-Mora, J.; Siegwart, R.; Beardsley, P.~\cite{Alon}"&2014&Mobile&Urban&Gesture Recognition&&&1/many&Interacting\\
"Castellano, G.; Leite, I.; Pereira, A.; Martinho, C.; Paiva, A.; McOwan, P.W.~\cite{Cast}"&2014&Social&Domestic&Social Classification and Communication&&&1&Interacting\\
"Chen, L.; Dong, Z.; Gao, S.; Yuan, B.; Pei, M.~\cite{Chen}"&2014&Mobile&Urban&Robot Movement in Human Spaces&Gesture Recognition&&1&Interacting\\
"Do, H.M.; Mouser, C.; Liu, M.; Sheng, W.~\cite{Do, }"&2014&Mobile&Field&Robot Movement in Human Spaces&&&44199&Following\\
"Fujii, T.; Lee, J.H.; Okamoto, S.~\cite{Fuji}"&2014&Mobile&Urban&Robot Movement in Human Spaces&Gesture Recognition&&1&Interacting\\
"Hu, J.-S.; Wang, J.-J.; Ho, D.M.~\cite{Hu, }"&2014&Mobile&Urban&Robot Movement in Human Spaces&&&1&Following\\
"Miyoshi, K.; Konomura, R.; Hori, K.~\cite{Miyo}"&2014&Drone&Field&Robot Movement in Human Spaces&&&44228&Interacting\\
"Morato, C.; Kaipa, K.N.; Zhao, B.; Gupta, S.K.~\cite{Mora}"&2014&Fixed Manipulator&Industrial&Object Handover and Collaborative Actions&&&1&Approaching\\
"Munaro, M.; Menegatti, E.~\cite{Muna}"&2014&Mobile&Urban&Robot Movement in Human Spaces&&&1&Following\\
"Nguyen, Q.; Yun, S.-S.; Choi, J.~\cite{Nguy}"&2014&Mobile&Urban&Robot Movement in Human Spaces&&&1&Following\\
"Petric, T.; Gams, A.; Zlajpah, L.; Ude, A.; Morimoto, J.~\cite{Petr}"&2014&Fixed Manipulator&Industrial&Learning from Demonstration&Gesture Recognition&&1&Interacting\\
"Prediger, M.; Braun, A.; Marinc, A.; Kuijper, A.~\cite{Pred}"&2014&Mobile&Urban&Robot Movement in Human Spaces&&&1&Following\\
"Scheggi, S.; Morbidi, F.; Prattichizzo, D.~\cite{Sche}"&2014&Mobile&Field&Robot Movement in Human Spaces&&&43832&Following\\
"Shieh, M.-Y.; Hsieh, C.-Y.; Hsieh, T.-M.~\cite{Shie}"&2014&Social&Domestic&Social Classification and Communication&Gesture Recognition&&1&Interacting\\
"Shieh, M.Y.; Chiou, J.S.; Pai, N.S.; Li, J.H.~\cite{Shie}"&2014&&&&&&&\\
"Taheri, A.R.; Alemi, M.; Meghdari, A.; Pouretemad, H.R.; Basiri, N.M.~\cite{Tahe}"&2014&Social&Urban&Social Classification and Communication&Gesture Recognition&&1&Interacting\\
"Tseng, S.-H.; Hsu, Y.-H.; Chiang, Y.-S.; Wu, T.-Y.; Fu, L.-C.~\cite{Tsen}"&2014&Mobile&Urban&Social Classification and Communication&Robot Movement in Human Spaces&&many/1&Interacting\\
"Xu, D.; Wu, X.; Chen, Y.-L.; Xu, Y.~\cite{Xu, }"&2014&Mobile&Urban&Robot Movement in Human Spaces&Gesture Recognition&&1&Interacting\\
"Ali, B.; Ayaz, Y.; Jamil, M.; Gilani, S.O.; Muhammad, N.~\cite{Ali,}"&2015&Mobile&Urban&Robot Movement in Human Spaces&&&1&Following\\
"Canal, G.; Angulo, C.; Escalera, S.~\cite{Cana}"&2015&Mobile&Domestic&Robot Movement in Human Spaces&Gesture Recognition&&44198&Interacting\\
"Cech, J.; Mittal, R.; Deleforge, A.; Sanchez-Riera, J.; Alameda-Pineda, X.; Horaud, R.~\cite{Cech}"&2015&Social&Domestic&Social Classification and Communication&&&1&Interacting\\
"Cherubini, A.; Passama, R.; Fraisse, P.; Crosnier, A.~\cite{Cher}"&2015&Fixed Manipulator&Industrial&Object Handover and Collaborative Actions&&&1&Touching\\
"Choudhary, G.B.; Chethan, R.B.V.~\cite{Chou}"&2015&Fixed Manipulator&Domestic&Object Handover and Collaborative Actions&Gesture Recognition&&1&Interacting\\
"Cicirelli, G.; Attolico, C.; Guaragnella, C.; D'Orazio, T.~\cite{Cici}"&2015&Mobile&Urban&Robot Movement in Human Spaces&Gesture Recognition&&1&Interacting\\
"Fareed, M.M.F.M.; Akram, Q.I.; Anees, S.B.A.; Fakih, A.H.~\cite{Fare}"&2015&Mobile Manipulator&Domestic&Robot Movement in Human Spaces&Gesture Recognition&&1&Interacting\\
"Gao, X.; Zheng, M.; Meng, M.Q.-H.~\cite{Gao,}"&2015&Social&Domestic&Social Classification and Communication&Gesture Recognition&&1&Interacting\\
"Gupta, M.; Behera, L.; Subramanian, V.K.; Jamshidi, M.M.~\cite{Gupt}"&2015&Mobile&Urban&Robot Movement in Human Spaces&&&1&Following\\
"Jevtić, A.; Doisy, G.; Parmet, Y.; Edan, Y.~\cite{Jevt}"&2015&Mobile&Domestic&Robot Movement in Human Spaces&Gesture Recognition&&1&Interacting\\
"Katsuki, Y.; Yamakawa, Y.; Ishikawa, M.~\cite{Kats}"&2015&Fixed Manipulator&Domestic&Gesture Recognition&&&1&Following\\
"Lalejini, A.; Duckworth, D.; Sween, R.; Bethel, C.L.; Carruth, D.~\cite{Lale}"&2015&Mobile&Urban&Robot Movement in Human Spaces&Gesture Recognition&&1&Interacting\\
"Li, L.; Xu, Q.; Wang, G.S.; Yu, X.; Tan, Y.K.; Li, H.~\cite{Li, }"&2015&&&&&&&\\
"Pai, N.-S.; Chang, C.-Y.; Chen, P.-Y.; Liao, M.-Y.~\cite{Pai,}"&2015&&&&&&&\\
"Quintero, C.P.; Tatsambon, R.; Gridseth, M.; Jagersand, M.~\cite{Quin}"&2015&Fixed Manipulator&Industrial&Object Handover and Collaborative Actions&Gesture Recognition&&1&Interacting\\
"Saleh, S.; Berns, K.~\cite{Sale}"&2015&Social&Urban&Social Classification and Communication&Gesture Recognition&&1&Interacting\\
"Virčíkova, M.; Sinčák, P.~\cite{Virč}"&2015&Social&Domestic&Social Classification and Communication&Gesture Recognition&&1&Interacting\\
"Yang, Y.; Yan, H.; Dehghan, M.; Ang, M.H.~\cite{Yang}"&2015&Fixed Manipulator&Industrial&Object Handover and Collaborative Actions&Gesture Recognition&&1&Interacting\\
"Bayram, B.; Ince, G.~\cite{Bayr}"&2016&Mobile&Urban&Robot Movement in Human Spaces&&&1&Following\\
"Chen, L.; Zhou, M.; Shi, W.; Xu, Y.; Wu, J.; Liao, C.; Wu, M.; She, J.; Hirota, K.~\cite{Chen}"&2016&&&&&&&\\
"Christiernin, L.G.; Augustsson, S.~\cite{Chri}"&2016&Fixed Manipulator&Industrial&Object Handover and Collaborative Actions&Gesture Recognition&&1&Interacting\\
"Ehlers, K.; Brama, K.~\cite{Ehle}"&2016&Mobile&Urban&Robot Movement in Human Spaces&Gesture Recognition&&1&Interacting\\
"Hassan, M.S.; Khan, A.F.; Khan, M.W.; Uzair, M.; Khurshid, K.~\cite{Hass}"&2016&Mobile&Urban&Robot Movement in Human Spaces&&&1&Interacting\\
"Ikai, T.; Kamiya, S.; Ohka, M.~\cite{Ikai}"&2016&Fixed Manipulator&Industrial&Object Handover and Collaborative Actions&Gesture Recognition&&1&Touching\\
"Kahily, H.M.; Sudheer, A.P.~\cite{Kahi}"&2016&Mobile&Domestic&Robot Movement in Human Spaces&&&1&Following\\
"Ke, X.; Zhu, Y.; Yang, Y.; Xing, J.; Luo, Z.~\cite{Ke, }"&2016&Social&Domestic&Social Classification and Communication&&&1&Interacting\\
"Koppula, H.S.; Saxena, A.~\cite{Kopp}"&2016&Mobile Manipulator&Domestic&Robot Movement in Human Spaces&Object Handover and Collaborative Actions&&1&Interacting\\
"Koustoumpardis, P.N.; Chatzilygeroudis, K.I.; Synodinos, A.I.; Aspragathos, N.A.~\cite{Kous}"&2016&Fixed Manipulator&Industrial&Object Handover and Collaborative Actions&&&1&Touching\\
"Mollaret, C.; Mekonnen, A.A.; Pinquier, J.; Lerasle, F.; Ferrane, I.~\cite{Moll}"&2016&Mobile&Domestic&Robot Movement in Human Spaces&Social Classification and Communication&&1&Approaching\\
"Moreno, R.J.; Mauledoux, M.; Avilés, O.F.~\cite{More}"&2016&Fixed Manipulator&Industrial&Object Handover and Collaborative Actions&&&1&Approaching\\
"Nguyen, V.-T.; Tran, T.-H.; Le, T.-L.; Mullot, R.; Courboulay, V.~\cite{Nguy}"&2016&Mobile&Urban&Social Classification and Communication&Gesture Recognition&&1&Interacting\\
"Potdar, S.; Sawarkar, A.; Kazi, F.~\cite{Potd}"&2016&Social&Domestic&Learning from Demonstration&Gesture Recognition&&1&Interacting\\
"Ratul, A.U.; Ali, M.T.; Ahasan, R.~\cite{Ratu}"&2016&Social&Domestic&Social Classification and Communication&&&1&Interacting\\
"Talebpour, Z.; Navarro, I.; Martinoli, A.~\cite{Tale}"&2016&Mobile&Domestic&Robot Movement in Human Spaces&&&1&Following\\
"Vasconcelos, P.A.A.; Pereira, H.N.S.; Macharet, D.G.; Nascimento, E.R.~\cite{Vasc}"&2016&Mobile&Urban&Robot Movement in Human Spaces&&&1&Avoiding\\
"Vaufreydaz, D.; Johal, W.; Combe, C.~\cite{Vauf}"&2016&Mobile&Domestic&Robot Movement in Human Spaces&&&1&Interacting\\
"Zhang, L.; Vaughan, R.~\cite{Zhan}"&2016&Mobile&Urban&Robot Movement in Human Spaces&&&1&Interacting\\
"Zhuang, C.; Zhou, H.; Sakane, S.~\cite{Zhua}"&2016&Social&Domestic&Learning from Demonstration&Action Recognition&&1&Interacting\\
"Angonese, A.T.; Ferreira Rosa, P.F.~\cite{Ango}"&2017&Mobile&Urban&Robot Movement in Human Spaces&&&1&Following\\
"Arenas, J.O.P.; Beleno, R.D.H.; Moreno, R.J.~\cite{Aren}"&2017&Fixed Manipulator&Industrial&Object Handover and Collaborative Actions&Gesture Recognition&&1&Interacting\\
"Bellarbi, A.; Kahlouche, S.; Achour, N.; Ouadah, N.~\cite{Bell}"&2017&Mobile&Urban&Robot Movement in Human Spaces&&&1&Avoiding\\
"Bilac, M.; Chamoux, M.; Lim, A.~\cite{Bila}"&2017&Social&Urban&Social Classification and Communication&&&1&Interacting\\
"Deepan Raj, M.; Gogul, I.; Thangaraja, M.; Kumar, V.S.~\cite{Deep}"&2017&Fixed Manipulator&Industrial&Object Handover and Collaborative Actions&Gesture Recognition&&1&Interacting\\
"Dometios, A.C.; Papageorgiou, X.S.; Arvanitakis, A.; Tzafestas, C.S.; Maragos, P.~\cite{Dome}"&2017&Fixed Manipulator&Domestic&Object Handover and Collaborative Actions&&&1&Touching\\
"Ghandour, M.; Liu, H.; Stoll, N.; Thurow, K.~\cite{Ghan}"&2017&Mobile&Urban&Robot Movement in Human Spaces&Gesture Recognition&&1&Interacting\\
"Görer, B.; Salah, A.A.; Akın, H.L.~\cite{Göre}"&2017&Mobile&Domestic&Social Classification and Communication&Gesture Recognition&&1&Interacting\\
"Han, J.; Jang, W.; Jung, D.; Lee, E.C.~\cite{Han,}"&2017&Social&Domestic&Gesture Recognition&&&1&Interacting\\
"Ju, Z.; Ji, X.; Li, J.; Liu, H.~\cite{Ju, }"&2017&Mobile&Domestic&Gesture Recognition&&&1&Interacting\\
"Lee, J.; Ryoo, M.S.~\cite{Lee,}"&2017&Fixed Manipulator&Industrial&Object Handover and Collaborative Actions&Action Recognition&&1&Interacting\\
"Maurtua, I.; Fernández, I.; Tellaeche, A.; Kildal, J.; Susperregi, L.; Ibarguren, A.; Sierra, B.~\cite{Maur}"&2017&Fixed Manipulator&Industrial&Object Handover and Collaborative Actions&Gesture Recognition&&1&Interacting\\
"Meghdari, A.; Shouraki, S.B.; Siamy, A.; Shariati, A.~\cite{Megh}"&2017&Social&Domestic&Gesture Recognition&Gesture Recognition&&1&Interacting\\
"Shariatee, M.; Khosravi, H.; Fazl-Ersi, E.~\cite{Shar}"&2017&Fixed Manipulator&Industrial&Object Handover and Collaborative Actions&&&1&Avoiding\\
"Song, H.; Feng, W.; Guan, N.; Huang, X.; Luo, Z.~\cite{Song}"&2017&Fixed Manipulator&Industrial&Object Handover and Collaborative Actions&Gesture Recognition&&1&Interacting\\
"Tölgyessy, M.; Dekan, M.; Duchoň, F.; Rodina, J.; Hubinský, P.; Chovanec, L.~\cite{Tölg}"&2017&Mobile&Domestic&Robot Movement in Human Spaces&Gesture Recognition&&1&Interacting\\
"Vasquez, A.; Kollmitz, M.; Eitel, A.; Burgard, W.~\cite{Vasq}"&2017&Mobile&Urban&Robot Movement in Human Spaces&&&1&Approaching\\
"Wang, Y.; Ye, X.; Yang, Y.; Zhang, W.~\cite{Wang}"&2017&Fixed Manipulator&Industrial&Object Handover and Collaborative Actions&Action Recognition&&1&Interacting\\
"Yao, N.; Anaya, E.; Tao, Q.; Cho, S.; Zheng, H.; Zhang, F.~\cite{Yao,}"&2017&Drone&Field&Robot Movement in Human Spaces&&&1&Interacting\\
"Yoo, B.-S.; Kim, J.-H.~\cite{Yoo,}"&2017&Social&Domestic&Learning from Demonstration&&&1&Interacting\\
"Zhu, T.; Zhao, Q.; Wan, W.; Xia, Z.~\cite{Zhu,}"&2017&Social&Domestic&Social Classification and Communication&&&1&Interacting\\
"Araiza-Lllan, D.; De San Bernabe Clemente, A.~\cite{Arai}"&2018&Fixed Manipulator&Industrial&Object Handover and Collaborative Actions&&&1&Approaching\\
"Bolano, G.; Tanev, A.; Steffen, L.; Roennau, A.; Dillmann, R.~\cite{Bola}"&2018&Fixed Manipulator&Industrial&Object Handover and Collaborative Actions&&&1&Interacting\\
"Bothe, K.; Winkler, A.; Goldhahn, L.~\cite{Both}"&2018&Fixed Manipulator&Industrial&Object Handover and Collaborative Actions&&&1&Interacting\\
"Du, G.; Chen, M.; Liu, C.; Zhang, B.; Zhang, P.~\cite{Du, }"&2018&Fixed Manipulator&Industrial&Object Handover and Collaborative Actions&Learning from Demonstration&&1&Following\\
"Efthymiou, N.; Koutras, P.; Filntisis, P.P.; Potamianos, G.; Maragos, P.~\cite{Efth}"&2018&Social&Urban&Social Classification and Communication&Action Recognition&&1&Interacting\\
"Gong, J.; Wang, H.; Lu, Z.; Feng, N.; Hu, F.~\cite{Gong}"&2018&Social&Domestic&Social Classification and Communication&&&1&Interacting\\
"Gui, L.-Y.; Zhang, K.; Wang, Y.-X.; Liang, X.; Moura, J.M.F.; Veloso, M.~\cite{Gui,}"&2018&Social&Domestic&Social Classification and Communication&Action Recognition&&1&Interacting\\
"Hong, C.; Chen, Z.; Zhu, J.; Zhang, X.~\cite{Hong}"&2018&Fixed Manipulator&Industrial&Object Handover and Collaborative Actions&&&1&Interacting\\
"Kalidolda, N.; Sandygulova, A.~\cite{Kali}"&2018&Social&Urban&Social Classification and Communication&Gesture Recognition&&1&Interacting\\
"Lavanya, K.N.; Shree, D.R.; Nischitha, B.R.; Asha, T.; Gururaj, C.~\cite{Lava}"&2018&Mobile&Domestic&Robot Movement in Human Spaces&Gesture Recognition&&1&Interacting\\
"Lee, H.; McCrink, M.H.; Gregory, J.W.~\cite{Lee,}"&2018&&&&&&&\\
"Li, X.; Cheng, H.; Ji, G.; Chen, J.~\cite{Li, }"&2018&Fixed Manipulator&Industrial&Learning from Demonstration&Object Handover and Collaborative Actions&&1&Following\\
"Long, Y.; Xu, Y.; Xiao, Z.; Shen, Z.~\cite{Long}"&2018&Mobile&Urban&Robot Movement in Human Spaces&Gesture Recognition&&1&Interacting\\
"Mao, L.; Zhu, P.~\cite{Mao,}"&2018&Mobile&Domestic&Robot Movement in Human Spaces&Gesture Recognition&&1&Approaching\\
"Pasinetti, S.; Nuzzi, C.; Lancini, M.; Sansoni, G.; Docchio, F.; Fornaser, A.~\cite{Pasi}"&2018&Fixed Manipulator&Industrial&Object Handover and Collaborative Actions&&&1&Avoiding\\
"Pentiuc, S.-G.; Vultur, O.-M.~\cite{Pent}"&2018&Mobile&Urban&Robot Movement in Human Spaces&Gesture Recognition&&1&Interacting\\
"Sorostinean, M.; Tapus, A.~\cite{Soro}"&2018&Social&Domestic&Social Classification and Communication&Action Recognition&&1&Interacting\\
"Weber, T.; Triputen, S.; Danner, M.; Braun, S.; Schreve, K.; Rätsch, M.~\cite{Webe}"&2018&Mobile&Urban&Robot Movement in Human Spaces&&&1&Following\\
"Yang, G.; Lv, H.; Chen, F.; Pang, Z.; Wang, J.; Yang, H.; Zhang, J.~\cite{Yang}"&2018&Fixed Manipulator&Domestic&Robot Movement in Human Spaces&Object Handover and Collaborative Actions&Gesture Recognition&1&Touching / carrying\\
"Yuan, W.; Li, Z.~\cite{Yuan}"&2018&Mobile&Urban&Robot Movement in Human Spaces&Gesture Recognition&&1&Following\\
"Zhang, K.; Zhang, L.~\cite{Zhan}"&2018&Mobile&Urban&Robot Movement in Human Spaces&&&1&Following / avoiding\\
"Zhang, L.; Zhang, K.~\cite{Zhan}"&2018&Mobile&Urban&Robot Movement in Human Spaces&Gesture Recognition&&1&Interacting\\
"Zhang, Z.; Chen, Z.; Li, W.~\cite{Zhan}"&2018&Mobile&Domestic&Robot Movement in Human Spaces&Gesture Recognition&&1&Touching\\
"Cazzato, D.; Cimarelli, C.; Sanchez-Lopez, J.L.; Olivares-Mendez, M.A.; Voos, H.~\cite{Cazz}"&2019&Social&Urban&Social Classification and Communication&&&1&Interacting\\
"Chalvatzaki, G.; Papageorgiou, X. S.; Maragos, P.; Tzafestas, C. S.~\cite{Chal}"&2019&Mobile&Domestic&Robot Movement in Human Spaces&&&1&Touching\\
"Chen, F.; Lv, H.; Pang, Z.; Zhang, J.; Hou, Y.; Gu, Y.; Yang, H.; Yang, G.~\cite{Chen}"&2019&Fixed Manipulator&Industrial&Object Handover and Collaborative Actions&Gesture Recognition&&1&Interacting\\
"Chen, J.; Kim, W.-J.~\cite{Chen}"&2019&Mobile&Urban&Robot Movement in Human Spaces&Gesture Recognition&&1&Interacting\\
"Chien, J.-C.; Dang, Z.-Y.; Lee, J.-D.~\cite{Chie}"&2019&Mobile&Urban&Robot Movement in Human Spaces&&&1&Following / avoiding\\
"Condés, I.; Cañas, J.M.~\cite{Cond}"&2019&Mobile&Domestic&Robot Movement in Human Spaces&&&1&Following\\
"Fang, J.; Qiao, M.; Pei, Y.~\cite{Fang}"&2019&Mobile&Urban&Robot Movement in Human Spaces&Gesture Recognition&&1&Interacting\\
"Haghighi, A.; Bdiwi, M.; Putz, M.~\cite{Hagh}"&2019&Fixed Manipulator&Industrial&Object Handover and Collaborative Actions&&&1&Interacting\\
"Jarosz, M.; Nawrocki, P.; Placzkiewicz, L.; Sniezynski, B.; Zielinski, M.; Indurkhya, B.~\cite{Jaro}"&2019&Social&Urban&Social Classification and Communication&&&1&Interacting\\
"Kogkas, A.; Ezzat, A.; Thakkar, R.; Darzi, A.; Mylonas, G.~\cite{Kogk}"&2019&Fixed Manipulator&Urban&Object Handover and Collaborative Actions&&&1&Touching\\
"Landi, C.T.; Cheng, Y.; Ferraguti, F.; Bonfe, M.; Secchi, C.; Tomizuka, M.~\cite{Land}"&2019&Fixed Manipulator&Industrial&Object Handover and Collaborative Actions&&&1&Avoiding\\
"Li, K.; Sun, S.; Zhao, X.; Wu, J.; Tan, M.~\cite{Li, }"&2019&Mobile&Urban&Robot Movement in Human Spaces&&&Several / 1&Approaching\\
"Li, K.; Wu, J.; Zhao, X.; Tan, M.~\cite{Li, }"&2019&Mobile&Urban&Robot Movement in Human Spaces&Action Recognition&&1&Interacting\\
"Li, T.-H.S.; Kuo, P.-H.; Tsai, T.-N.; Luan, P.-C.~\cite{Li, }"&2019&Social&Urban&Social Classification and Communication&&&1&Interacting\\
"Lima, B.; Júnior, G.L.N.; Amaral, L.; Vieira, T.; Ferreira, B.; Vieira, T.~\cite{Lima}"&2019&Fixed Manipulator&Industrial&Object Handover and Collaborative Actions&Gesture Recognition&&1&Interacting\\
"Luo, X.; Amighetti, A.; Zhang, D.~\cite{Luo,}"&2019&Mobile Manipulator&Urban&Robot Movement in Human Spaces&Gesture Recognition&&1&Interacting\\
"Luo, X.; Zhang, D.; Jin, X.~\cite{Luo,}"&2019&Mobile&Domestic&Robot Movement in Human Spaces&&&1&Following\\
"Martin, J.B.; Moutarde, F.~\cite{Mart}"&2019&Fixed Manipulator&Industrial&Object Handover and Collaborative Actions&Gesture Recognition&&1&Interacting\\
"Mazhar, O.; Navarro, B.; Ramdani, S.; Passama, R.; Cherubini, A.~\cite{Mazh}"&2019&Fixed Manipulator&Industrial&Object Handover and Collaborative Actions&Gesture Recognition&&many/1&Touching\\
"Miller, J.; Hong, S.; Lu, J.~\cite{Mill}"&2019&Mobile&Urban&Robot Movement in Human Spaces&Gesture Recognition&&1&Interacting\\
"Moh, J.J.; Kijima, T.; Zhang, B.; Lim, H.-O.~\cite{Moh,}"&2019&Mobile Manipulator&Domestic&Robot Movement in Human Spaces&Gesture Recognition&Object Handover and Collaborative Actions&1&Interacting\\
"Scimmi, L.S.; Melchiorre, M.; Mauro, S.; Pastorelli, S.~\cite{Scim}"&2019&Fixed Manipulator&Industrial&Object Handover and Collaborative Actions&&&1&Touching\\
"Sriram, K.N.V.; Palaniswamy, S.~\cite{Srir}"&2019&Mobile Manipulator&Domestic&Object Handover and Collaborative Actions&Object Handover and Collaborative Actions&Gesture Recognition&1&Touching\\
"Valle, A.F.; Alenyà, G.; Chance, G.; Caleb-Solly, P.; Dogramadzi, S.; Torras, C.~\cite{Vall}"&2019&Fixed Manipulator&Domestic&Object Handover and Collaborative Actions&&&1&Touching\\
"Vysocký, A.; Pastor, R.; Novák, P.~\cite{Vyso}"&2019&Fixed Manipulator&Industrial&Object Handover and Collaborative Actions&Gesture Recognition&&1&Interacting\\
"Wong, C.-C.; Chen, H.-C.; Lee, C.-T.; Wang, C.-C.; Feng, H.-M.~\cite{Wong}"&2019&&&&&&&\\
"Wu, Y.; Yang, Q.; Zhou, X.~\cite{Wu, }"&2019&&&&&&&\\
"Yamakawa, Y.; Matsui, Y.; Ishikawa, M.~\cite{Yama}"&2019&Fixed Manipulator&Industrial&Object Handover and Collaborative Actions&&&1&Touching\\
"Yang, C.-T.; Zhang, T.; Chen, L.-P.; Fu, L.-C.~\cite{Yang}"&2019&Mobile&Urban&Robot Movement in Human Spaces&&&1&Avoiding\\
"Zardykhan, D.; Svarny, P.; Hoffmann, M.; Shahriari, E.; Haddadin, S.~\cite{Zard}"&2019&Fixed Manipulator&Industrial&Object Handover and Collaborative Actions&&&1&Avoiding\\
"Zhang, M.; Liu, X.; Xu, D.; Cao, Z.; Yu, J.~\cite{Zhan}"&2019&Mobile&Urban&Robot Movement in Human Spaces&&&1&Following\\
"Zhao, R.; Sidobre, D.~\cite{Zhao}"&2019&&&&&&&\\
"Anuradha, U.A.D.N.; Kumari, K.W.S.N.; Chathuranga, K.W.S.~\cite{Anur}"&2020&Mobile&Urban&Robot Movement in Human Spaces&Robot Movement in Human Spaces&&1&Following\\
"Arai, K.~\cite{Arai}"&2020&Fixed Manipulator&Domestic&Object Handover and Collaborative Actions&&&1&Touching\\
"Augello, A.; Ciulla, A.; Cuzzocrea, A.; Gaglio, S.; Pilato, G.; Vella, F.~\cite{Auge}"&2020&Social&Urban&Social Classification and Communication&&&1&Interacting\\
"Avioz-Sarig, O.; Olatunji, S.; Sarne-Fleischmann, V.; Edan, Y.~\cite{Avio}"&2020&Social&Domestic&Social Classification and Communication&Gesture Recognition&&1&Interacting\\
"Bingol, M.C.; Aydogmus, O.~\cite{Bing}"&2020&&&&&&&\\
"Chan, C.-C.; Tsai, C.-C.~\cite{Chan}"&2020&Fixed Manipulator&Industrial&Object Handover and Collaborative Actions&&&1&Avoiding\\
"Ferraguti, F.; Talignani Landi, C.; Costi, S.; Bonfè, M.; Farsoni, S.; Secchi, C.; Fantuzzi, C.~\cite{Ferr}"&2020&Fixed Manipulator&Industrial&Object Handover and Collaborative Actions&&&1&Touching\\
"Gao, Q.; Liu, J.; Ju, Z.~\cite{Gao,}"&2020&Fixed Manipulator&Domestic&Gesture Recognition&&&1&Interacting\\
"Hwang, C.-L.; Wang, D.-S.; Weng, F.-C.; Lai, S.-L.~\cite{Hwan}"&2020&Mobile&Urban&Robot Movement in Human Spaces&&&1&Following\\
"Lang, X.; Feng, Z.; Yang, X.~\cite{Lang}"&2020&Social&Urban&Action Recognition&Social Classification and Communication&&1&Interacting\\
"Lee, C.-Y.; Lee, H.; Hwang, I.; Zhang, B.-T.~\cite{Lee,}"&2020&Mobile Manipulator&Domestic&Robot Movement in Human Spaces&Object Handover and Collaborative Actions&&Several/1&Approaching\\
"Lee, J.; Ahn, B.~\cite{Lee,}"&2020&Mobile&Urban&Robot Movement in Human Spaces&&&1&Following\\
"Liu, Z.; Wang, X.; Cai, Y.; Xu, W.; Liu, Q.; Zhou, Z.; Pham, D.T.~\cite{Liu,}"&2020&Fixed Manipulator&Industrial&Object Handover and Collaborative Actions&&&1&Avoiding\\
"Lu, G.; Tang, W.; Zheng, J.; Chen, T.; Zou, X.~\cite{Lu, }"&2020&Social&Domestic&Gesture Recognition&&&1&Interacting\\
"Mronga, D.; Knobloch, T.; de Gea Fernández, J.; Kirchner, F.~\cite{Mron}"&2020&Fixed Manipulator&Industrial&Object Handover and Collaborative Actions&&&1&Avoiding\\
"Phong, N.T.T.; Nam, L.H.T.; Thinh, N.T.~\cite{Phon}"&2020&Mobile&Urban&Social Classification and Communication&&&1&Interacting\\
"Tarbouriech, S.; Suleiman, W.~\cite{Tarb}"&2020&Fixed Manipulator&Industrial&Object Handover and Collaborative Actions&&&1&Interacting\\
"Van Den Broek, M.K.; Moeslund, T.B.~\cite{Van }"&2020&Fixed Manipulator&Industrial&Object Handover and Collaborative Actions&&&1&Touching\\
"Waskito, T.B.; Sumaryo, S.; Setianingsih, C.~\cite{Wask}"&2020&Mobile&Domestic&Robot Movement in Human Spaces&Gesture Recognition&&1&Interacting\\
"Wu, Z.; Payandeh, S.~\cite{Wu, }"&2020&Mobile&Urban&Robot Movement in Human Spaces&&&1&Following\\
"Xu, J.; Li, J.; Zhang, S.; Xie, C.; Dong, J.~\cite{Xu, }"&2020&Mobile&Urban&Robot Movement in Human Spaces&Gesture Recognition&&1&Interacting\\
"Yuan, X.; Dai, S.; Fang, Y.~\cite{Yuan}"&2020&Social&Domestic&Social Classification and Communication&Gesture Recognition&&1&Interacting\\
"Zhang, J.; Li, P.; Zhu, T.; Zhang, W.-A.; Liu, S.~\cite{Zhan}"&2020&Fixed Manipulator&Industrial&Object Handover and Collaborative Actions&&&1&Touching\\

\bottomrule
\end{tabular}
\end{table}
